Function based sim-to-real learning for shape control of deformable free-form surfaces

For the shape control of deformable free-form surfaces, simulation plays a crucial role in establishing the mapping between the actuation parameters and the deformed shapes. The differentiation of this forward kinematic mapping is usually employed to solve the inverse kinematic problem for determining the actuation parameters that can realize a target shape. However, the free-form surfaces obtained from simulators are always different from the physically deformed shapes due to the errors introduced by hardware and the simplification adopted in physical simulation. To fill the gap, we propose a novel deformation function based sim-to-real learning method that can map the geometric shape of a simulated model into its corresponding shape of the physical model. Unlike the existing sim-to-real learning methods that rely on completely acquired dense markers, our method accommodates sparsely distributed markers and can resiliently use all captured frames -- even for those in the presence of missing markers. To demonstrate its effectiveness, our sim-to-real method has been integrated into a neural network-based computational pipeline designed to tackle the inverse kinematic problem on a pneumatically actuated deformable mannequin.

==> tex/Alg.tex <==
\begin{algorithm}[t]
\caption{FastIK Solver}%DeepSurfIK
\label{algInverseKinematic}
\LinesNumbered

\KwIn{The target shape $\mathcal{T}$, the initial actuation $\mathbf{a}_0$, the initial transformation matrix $T_{0}$, minimum step size threshold $h_{min}$, relative objective function value decreasing threshold $\lambda$ and the maximally allowed iterations $i_{max}$.}

% \KwOut{The optimized actuation $\mathbf{a}_{opt}$, the pose of $\mathcal{T}_{opt}$ as $(\mathbf{R}_{opt},{t}_{opt})$ and the resultant shape $\mathcal{S}_{opt}$.} 


\KwOut{The optimized actuation $\mathbf{a}_{opt}$} 



Set $i = 0$ and apply the initial actuation vector $\mathbf{a_0}$;

Apply initial transformation $T_{0}$ to target model $\mathcal{T}$;

%Evaluate the objective function $D_0 =D(\mathbf{a}_{0})$; 

Set initial objective function relative decreasing percentage $r_0 = 1.0$;



\While{$i<i_{max}$ and $r_{i}>\lambda$}
{
    \tcc{Calculate new transformation}
    ICP-based pose estimation to get $T_{i}$ that is applied on $\mathcal{T}$ to better align with $\mathcal{S}_{i}$;

    Evaluate the objective function $D_i =D(\mathbf{a}_{i})$;

    \tcc{Gradient-based iteration with transformation fixed}
    \While{True}
    {
    
    Compute the gradient of $D(\mathbf{a}_{i})$ as $\nabla D$ by differentiating neural deformation model;

    Compute optimal step size $h$ by soft line search method \cite{Guoxin2020TRO};

    \If{$h \leqslant h_{min}$}
    {
        break;
    }
    
    
    Set $\mathbf{a}_{i+1} = \mathbf{a}_{i} - h \nabla D$ and $i=i+1$;


    Evaluate the objective function $D_i = D(\mathbf{a}_{i})$; 


    Evaluate the objective function relative decreasing percentage as: $r_{i} =\frac{\abs{D_{i}-D_{i-1}}}{\abs{D_{i}}}$;

     \If{$r_{i} \leqslant \lambda$}
    {
        break;
     }
    
    }
}
$\mathbf{a}_{opt} = \mathbf{a}_{i}$;


\KwRet{$\mathbf{a}_{opt}$};
%\label{bla}

\end{algorithm}

% \begin{algorithm}[h]
% \caption{FastIK Solver}%DeepSurfIK
% \label{algInverseKinematic}
% \LinesNumbered

% \KwIn{The target shape $\mathcal{T}$, the initial actuation $\mathbf{a}_0$, the initial transformation matrix $T_{0}$, relative objective function value decreasing threshold $\lambda$ and the maximally allowed iterations $i_{max}$.}

% \KwOut{The optimized actuation $\mathbf{a}_{opt}$, the pose of $\mathcal{T}_{opt}$ as $(\mathbf{R}_{opt},{t}_{opt})$ and the resultant shape $\mathcal{S}_{opt}$.} 


% Set $i = 0$ and apply the initial actuation vector $\mathbf{a_0}$;

% Evaluate the objective function $\mathcal{O}_0 =\mathcal{O}(\mathbf{a}_{0})$; 

% Initialize objective function relative decreasing percentage $\mathcal{D}_0 = 1.0$;



% \While{$i<i_{max}$}
% {
%     \tcc{Calculate new transformation}
%     ICP-based pose estimation to get $T_{i}$ that is applied on $\mathcal{T}$ to better align with $\mathcal{S}_{i}$;

%     \tcc{Gradient-based iteration with transformation fixed}
%     \While{$\mathcal{D}_{i} > \lambda$ and $i<i_{max}$}
%     {
    
%     Compute the gradient of $D(\mathbf{a}_{i})$ as $\nabla D$ by differentiating neural deformation model;
    
%     Set the step size $\Delta h=1.0$;
    
%     Set $\mathcal{O}_{origin} = \mathcal{O}_{i}$
    
%     \tcc{Soft line-search}
    
%     \tcc{Step 1: Shrinking}
    
    
%     \Repeat{$\mathcal{O}_{shrink} < \mathcal{O}_{origin}$}
%     {
%         $\mathcal{O}_{shrink} = \mathcal{O}(\mathbf{a}_{i} + \Delta h \nabla \mathcal{O})$;
        
%         $\Delta h = \tau * \Delta h$;
    
%     }
%     $\mathcal{O}_{opt} = \mathcal{O}_{shrink}$;
    
    
%     \tcc{Step 2: Expanding}
%     Set $h= \Delta h$;
    
%     \Repeat{$\mathcal{O}_{expand} > \mathcal{O}_{opt}$}
%     {
    
%     Compute and update $\mathcal{O}_{expand}=\mathcal{O}(\mathbf{a}_{i} + (h + \Delta h)\nabla \mathcal{O})$;
    
%     \If{$\mathcal{O}_{expand} \leq \mathcal{O}_{opt}$}
%     {
%     Set $\mathcal{O}_{opt} = \mathcal{O}_{expand}$ and $h = h + \Delta h$;
%     }
    
%     }
    
    
%     \tcc{Best $h$ has been found}
    
%     Set $\mathbf{a}_{i+1} = \mathbf{a}_{i} + h \nabla \mathcal{O}$ and $i=i+1$;

%     \tcc{Ready to get into next iteration}
%     Evaluate the objective function $\mathcal{O}_i = \mathcal{O}(\mathbf{a}_{i})$; 

%     Evaluate the objective function relative decreasing percentage as: $\mathcal{D}_{i} =\frac{\abs{\mathcal{O}_{i}-\mathcal{O}_{i-1}}}{\abs{\mathcal{O}_{i}}}$;

    
    
%     }
% }
% \KwRet{$\mathbf{a}_{opt}$};
% %\label{bla}

% \end{algorithm}

==> tex/TableI.tex <==

\begin{table*}[t]
  \centering
    %%%%%%%%%%%%%Second include the Table
\small %\small \footnotesize %scriptsize %\tiny 
\caption{Field Learning Architecture Comparison}\label{tab:fieldLearningComparison}
\begin{tabular}{c|c|c|c||c|c|c|c|c|c|c}  %adjust column number 
\hline \hline                       % two horizontal line
%\specialrule{0em}{2pt}{1pt}         %vertical space
\multicolumn{2}{c|}{\multirow{2}{*}{Learning Architecture}}  & 
% \multicolumn{1}{c|}{\multirow{2}{*}{Type}} &
\multicolumn{2}{c|}{Case \Romannum{1}$^\dagger$} & %Case \Romannum{1}
\multicolumn{2}{c|}{Case \Romannum{2}} &
\multicolumn{2}{c|}{Case \Romannum{3}} &
% \multicolumn{2}{c|}{Case \Romannum{5}} &
\multicolumn{1}{c|}{\multirow{2}{*}{Type \Romannum{1}$^\ddagger$}} &   %$C^{1}$ Continuity
\multicolumn{1}{c|}{\multirow{2}{*}{Type \Romannum{2}$^\star$}} &   %Smoothness
\multicolumn{1}{c}{\multirow{2}{*}{Type \Romannum{3}$^\ast$}} \\ %Small Reality Gap
%\hline
\cline{3-8}
\multicolumn{2}{c|}{}  & 

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

% \multicolumn{1}{c|}{Mean} &  %Mean Error
% \multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{} &   %$C^{1}$ Continuity
\multicolumn{1}{c|}{} &   %Smoothness
\multicolumn{1}{c}{} \\

\hline\hline

%\color{blue}\ding{51} & \color{red}\ding{55}
\multicolumn{1}{c|}{\multirow{4}{*}{Naive Field Network}}  & 
\multicolumn{1}{c|}{(A) Recon. + ReLU}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c}{NA}  \\
\cline{2-11}

\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(B) Recon. + Lip.\,\,\,}  & 
% \multicolumn{1}{c|}{2.53}  & 
% \multicolumn{1}{c|}{11.86}  & 

\multicolumn{1}{c|}{4.32}  & 
\multicolumn{1}{c|}{24.36}  & 

\multicolumn{1}{c|}{3.01}  & 
\multicolumn{1}{c|}{21.93}  & 

\multicolumn{1}{c|}{3.61}  & 
\multicolumn{1}{c|}{32.79}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}   \\
\cline{2-11}


\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(C) Recon. + Siren}  & 
% \multicolumn{1}{c|}{\color{blue}2.14}  & 
% \multicolumn{1}{c|}{\color{blue}9.33}  & 

\multicolumn{1}{c|}{4.97}  & 
\multicolumn{1}{c|}{24.67}  & 

\multicolumn{1}{c|}{4.02}  & 
\multicolumn{1}{c|}{15.88}  & 

\multicolumn{1}{c|}{4.25}  & 
\multicolumn{1}{c|}{17.99}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}  \\
\cline{2-11}

\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(D) Recon. + RBF}  & 
% \multicolumn{1}{c|}{2.15}  & 
% \multicolumn{1}{c|}{10.26}  & 

\multicolumn{1}{c|}{7.09}  & 
\multicolumn{1}{c|}{24.80}  & 

\multicolumn{1}{c|}{3.96}  & 
\multicolumn{1}{c|}{15.32}  & 

\multicolumn{1}{c|}{3.75}  & 
\multicolumn{1}{c|}{19.65}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}  \\


\hline \hline   %segmentation line between naive filed & rbf field
\multicolumn{1}{c|}{RBF Field Network}  & 
\multicolumn{1}{c|}{(E)}  & 
% \multicolumn{1}{c|}{2.21}  & 
% \multicolumn{1}{c|}{11.63}  & 

\multicolumn{1}{c|}{\color{blue}4.13}  & 
\multicolumn{1}{c|}{\color{blue}18.70}  & 

\multicolumn{1}{c|}{\color{blue}2.96}  & 
\multicolumn{1}{c|}{\color{blue}14.53}  & 

\multicolumn{1}{c|}{\color{blue}3.57}  & 
\multicolumn{1}{c|}{\color{blue}16.26}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{blue}\ding{51}}  \\
\hline\hline
\end{tabular}
\begin{flushleft}\footnotesize
$^\ddagger$ $C^1$ Continuity: measure whether the shape gradient is continuous on the surface.\\
$^\star$ Local Shape Smoothness (defined by Eq.\ref{eqSmoothness}): measure whether the local shape is changing dramatically.\\
$^\ast$ Small Reality Gap: measure the ability of the specific Sim2Real transfer to reduce error.\\
$^\dagger$ Case I: Apply actuation I to deform the prototype.
Mean and Max.: the mean and the maximum error of the calibrated model to the scanned one.\\
\end{flushleft}


%vertical space
\vspace*{0.0\floatsep}

%%%%%%%%%%%%%Then include Figure
\begingroup
\includegraphics[width=1.0\linewidth]{fig/figFieldPropertyComp.jpg}\\
\captionof{figure}{Experiments to compare the output of different field networks: The first one is to measure the $C^1$ Continuity (Type I) and shape smoothness (Type II). All five baselines and our proposed methods are tested and visualized in  (a). Furthermore, we have tested the ability of different methods to reduce the reality gap (Type III) by measuring their distance to the scanned model and visualizing the error by colormap (red color is 15mm). Three different actuation parameters are applied and the results are illustrated from Case I to Case III (b-d). The mean errors and maximum errors are listed in Table.~\ref{tab:fieldLearningComparison}. In conclusion, our proposed method is the only one to simultaneously satisfy all three requirements.
\Tian{Need Case I to be improved}}\label{figFieldProperty}
\endgroup

% Experiments to test the $C^1$ continuity, smoothness a of the learned field from different field learning networks: (a) (b) (c)}

\end{table*}


==> tex/TableTimes.tex <==

\begin{table}[t]
  \centering

\begingroup
\includegraphics[width=1.0\linewidth]{fig/figSim2RealDataset.jpg}\\
\vspace*{-0.5\floatsep}
\captionof{figure}{
The training dataset for our Sim2Real network only consists of 43 frames. What's more, there exist information loss in some frames as indicated by the red dash line, which can be successfully handled by our Robust field learning framework. What's more, our framework can use only sparse ground-truth information (sparse markers compared to dense control points as surface descriptors) to bridge the reality gap as shown in blue line.
}\label{figDataset}
\endgroup
\vspace*{1.0\floatsep}










  
    %%%%%%%%%%%%%Second include the Table
\footnotesize %\small \footnotesize %scriptsize %\tiny 
%Computation time for a single gradient evaluation of the RBF Field Network. 
\caption{The computation cost (unit: millisecond) of the single shape approximation loss $D$ calculation and its gradient $\frac{\partial D}{\partial \textbf{a}}$ (with respect to actuation $\textbf{a}$) evaluation is collected, which is broken down into seven distinct operations (details are listed in Appendix.\ref{Appendix:GradCompShapeLoss} \& \ref{Appendix:GradCompNerualDef} and Fig.~\ref{figVarRelation}). Note that n is the number of the resampling points on the surface and we chose it to be 1200.
}\label{tab:rbfFieldCompTime}
\begin{tabular}{c|c|c|c|c|c|c|c}  %adjust column number 
\hline \hline                       % two horizontal line
%\specialrule{0em}{2pt}{1pt}         %vertical space
\multicolumn{1}{c|}{\multirow{2}{*}{Type}$^\ast$}  & 
\multicolumn{3}{c|}{Forward Pass$^\dagger$} & 
\multicolumn{3}{c|}{Back Propagation$^\ddagger$} &
\multicolumn{1}{c}{\multirow{2}{*}{Total}}\\ %Small Reality Gap
%\hline

% $^\dagger$ \\
% $^\ddagger$ \\
% $^\star$ \\
% $^\ast$ \\

\cline{2-7}
\multicolumn{1}{c|}{}  & 

\multicolumn{1}{c|}{Times} &  %Mean Error
\multicolumn{1}{c|}{Time} &  %Max. Error
\multicolumn{1}{c|}{Total} &  %Mean Error

\multicolumn{1}{c|}{Times} &  %Max. Error
\multicolumn{1}{c|}{Time} &  %Mean Error
\multicolumn{1}{c|}{Total} &
\multicolumn{1}{c}{}\\
\hline\hline

%first operator
\multicolumn{1}{c|}{\Romannum{1}}  & 

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{11.2} &  
\multicolumn{1}{c|}{11.2} & 

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{22.5} & 
\multicolumn{1}{c|}{22.5} & 
\multicolumn{1}{c}{33.7}\\

%second operator
\hline
\multicolumn{1}{c|}{\Romannum{2}}  & 

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{1.3} &  
\multicolumn{1}{c|}{1.3} &  

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{2.1} & 
\multicolumn{1}{c|}{2.1} & 
\multicolumn{1}{c}{3.4}\\

%third operator
\hline
\multicolumn{1}{c|}{\Romannum{3}}  & 

\multicolumn{1}{c|}{n} &  
\multicolumn{1}{c|}{1.1e-2} &  
\multicolumn{1}{c|}{12.8} & 

\multicolumn{1}{c|}{n} &  
\multicolumn{1}{c|}{1.0e-2} &  
\multicolumn{1}{c|}{12.4} & 
\multicolumn{1}{c}{25.2}\\

%fourth operator
\hline
\multicolumn{1}{c|}{\Romannum{4}}  & 

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{1.6} &  
\multicolumn{1}{c|}{1.6} & 

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{1.5} &  
\multicolumn{1}{c|}{1.5} & 
\multicolumn{1}{c}{3.1}\\

%fifth operator
\hline
\multicolumn{1}{c|}{\Romannum{5}}  & 

\multicolumn{1}{c|}{\multirow{3}{*}{n}} & 
\multicolumn{1}{c|}{\multirow{3}{*}{7.5e-4}} & 
\multicolumn{1}{c|}{\multirow{3}{*}{0.9}} & 

\multicolumn{1}{c|}{n} &  
\multicolumn{1}{c|}{2.0e-3} & 
\multicolumn{1}{c|}{2.4} & 
\multicolumn{1}{c}{\multirow{3}{*}{17.0}}\\

%sixth operator
\cline{1-1}
\cline{5-7}
\multicolumn{1}{c|}{\Romannum{6}}  & 

\multicolumn{1}{c|}{} &  %empty
\multicolumn{1}{c|}{} &  %empty
\multicolumn{1}{c|}{} &  %empty

\multicolumn{1}{c|}{n} &  
\multicolumn{1}{c|}{5.3e-3} &  
\multicolumn{1}{c|}{6.3} & 
\multicolumn{1}{c}{}\\

%seventh operator
\cline{1-1}
\cline{5-7}
\multicolumn{1}{c|}{\Romannum{7}}  & 

\multicolumn{1}{c|}{} &  %empty
\multicolumn{1}{c|}{} &  %empty
\multicolumn{1}{c|}{} &  %empty

\multicolumn{1}{c|}{n} &  
\multicolumn{1}{c|}{6.2e-3} &  
\multicolumn{1}{c|}{7.4} & 
\multicolumn{1}{c}{}\\

%Total 
\hline
\hline
\multicolumn{1}{c|}{Total$^\star$}  & 

\multicolumn{1}{c}{} &  
\multicolumn{1}{c|}{} &  
\multicolumn{1}{c|}{\color{red}27.8} & 

\multicolumn{1}{c}{} &  
\multicolumn{1}{c|}{} &  
\multicolumn{1}{c|}{\color{red}54.6} & 
\multicolumn{1}{c}{\color{blue}82.4}\\

\hline\hline
\end{tabular}
\begin{flushleft}\footnotesize
$^\ast$  The specific operation as detailed in Fig.~\ref{figVarRelation}.\\
$^\star$ The total time cost of the forward pass and backward pass.\\
$^\dagger$ Forward pass of the specific operation.\\
$^\ddagger$ Backward pass of the specific operation.\\


\end{flushleft}
% %Computation time for a single gradient evaluation of the RBF Field Network. 
% \caption{The computation cost (unit: millisecond) of the single shape approximation loss $D$ calculation and its gradient $\frac{\partial D}{\partial \textbf{a}}$ (with respect to actuation $\textbf{a}$) evaluation is collected, which is broken down into seven distinct operations (details are listed in Appendix.\ref{Appendix:GradCompShapeLoss} \& \ref{Appendix:GradCompNerualDef} and Fig.~\ref{figVarRelation}). Note that n is the number of the resampling points on the surface and we chose it to be 1200.
% }\label{tab:rbfFieldCompTime}

\end{table}


==> tex/backupFolder/tableBackup.tex <==
\begin{table*}[h] \footnotesize%\tiny %scriptsize
%\footnotesize
%special character: https://www-h.eng.cam.ac.uk/help/tpl/textprocessing/latex_advanced/node14.html

\centering
\begin{tabular}{c|c|c|c|c|c||c|c|c|c|c|c|c}  %adjust column number 
\hline \hline                       % two horizontal line
%\specialrule{0em}{2pt}{1pt}         %vertical space
\multicolumn{2}{c|}{\multirow{2}{*}{Learning Architecture}}  & 
% \multicolumn{1}{c|}{\multirow{2}{*}{Type}} &
\multicolumn{2}{c|}{Case \Romannum{1}$^\dagger$} & %Case \Romannum{1}
\multicolumn{2}{c|}{Case \Romannum{2}} &
\multicolumn{2}{c|}{Case \Romannum{3}} &
\multicolumn{2}{c|}{Case \Romannum{4}} &
% \multicolumn{2}{c|}{Case \Romannum{5}} &
\multicolumn{1}{c|}{\multirow{2}{*}{Type \Romannum{1}$^\ddagger$}} &   %$C^{1}$ Continuity
\multicolumn{1}{c|}{\multirow{2}{*}{Type \Romannum{2}$^\star$}} &   %Smoothness
\multicolumn{1}{c}{\multirow{2}{*}{Type \Romannum{3}$^\ast$}} \\ %Small Reality Gap
%\hline
\cline{3-10}
\multicolumn{2}{c|}{}  & 

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

% \multicolumn{1}{c|}{Mean} &  %Mean Error
% \multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{} &   %$C^{1}$ Continuity
\multicolumn{1}{c|}{} &   %Smoothness
\multicolumn{1}{c}{} \\

\hline\hline

%\color{blue}\ding{51} & \color{red}\ding{55}
\multicolumn{1}{c|}{\multirow{4}{*}{Naive Field Network}}  & 
\multicolumn{1}{c|}{(A)Recon.+ReLU}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c}{NA}  \\
\cline{2-13}

\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(B)Recon.+Lip.}  & 
\multicolumn{1}{c|}{2.53}  & 
\multicolumn{1}{c|}{11.86}  & 

\multicolumn{1}{c|}{4.32}  & 
\multicolumn{1}{c|}{24.36}  & 

\multicolumn{1}{c|}{3.01}  & 
\multicolumn{1}{c|}{21.93}  & 

\multicolumn{1}{c|}{3.61}  & 
\multicolumn{1}{c|}{32.79}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}   \\
\cline{2-13}


\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(C)Recon.+Siren}  & 
\multicolumn{1}{c|}{\color{blue}2.14}  & 
\multicolumn{1}{c|}{\color{blue}9.33}  & 

\multicolumn{1}{c|}{4.97}  & 
\multicolumn{1}{c|}{24.67}  & 

\multicolumn{1}{c|}{4.02}  & 
\multicolumn{1}{c|}{15.88}  & 

\multicolumn{1}{c|}{4.25}  & 
\multicolumn{1}{c|}{17.99}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}  \\
\cline{2-13} 

\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(D)Recon.+RBF}  & 
\multicolumn{1}{c|}{2.15}  & 
\multicolumn{1}{c|}{10.26}  & 

\multicolumn{1}{c|}{7.09}  & 
\multicolumn{1}{c|}{24.80}  & 

\multicolumn{1}{c|}{3.96}  & 
\multicolumn{1}{c|}{15.32}  & 

\multicolumn{1}{c|}{3.75}  & 
\multicolumn{1}{c|}{19.65}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}  \\


\hline \hline   %segmentation line between naive filed & rbf field
\multicolumn{1}{c|}{RBF Field Network}  & 
\multicolumn{1}{c|}{(E)}  & 
\multicolumn{1}{c|}{2.21}  & 
\multicolumn{1}{c|}{11.63}  & 

\multicolumn{1}{c|}{\color{blue}4.13}  & 
\multicolumn{1}{c|}{\color{blue}18.70}  & 

\multicolumn{1}{c|}{\color{blue}2.96}  & 
\multicolumn{1}{c|}{\color{blue}14.53}  & 

\multicolumn{1}{c|}{\color{blue}3.57}  & 
\multicolumn{1}{c|}{\color{blue}16.26}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{blue}\ding{51}}  \\
\hline\hline
\end{tabular}
%\footnotesize%\tiny %scriptsize
\begin{flushleft}\footnotesize
$^\ddagger$ $C^1$ Continuity: measure whether the shape gradient is continuous on the surface.\\
$^\star$ Local Shape Smoothness: measure whether the local shape is changing dramatically.\\
$^\ast$ Small Reality Gap: measure the ability of the specific Sim2Real transfer to reduce error.\\
$^\dagger$ Case I: Apply actuation I to deform the prototype.
Mean and Max.: the mean and the maximum error of the calibrated model to the scanned one.\\
\end{flushleft}

\caption{Field Learning Architecture Comparison}\label{tab:fieldLearningComparison}
\vspace{-10pt}
\end{table*}












































\begin{table*}
  \centering
    %%%%%%%%%%%%%Second include the Table
\footnotesize
\caption{Field Learning Architecture Comparison}\label{tab:fieldLearningComparison}
\begin{tabular}{c|c|c|c|c|c||c|c|c|c|c|c|c}  %adjust column number 
\hline \hline                       % two horizontal line
%\specialrule{0em}{2pt}{1pt}         %vertical space
\multicolumn{2}{c|}{\multirow{2}{*}{Learning Architecture}}  & 
% \multicolumn{1}{c|}{\multirow{2}{*}{Type}} &
\multicolumn{2}{c|}{Case \Romannum{1}$^\dagger$} & %Case \Romannum{1}
\multicolumn{2}{c|}{Case \Romannum{2}} &
\multicolumn{2}{c|}{Case \Romannum{3}} &
\multicolumn{2}{c|}{Case \Romannum{4}} &
% \multicolumn{2}{c|}{Case \Romannum{5}} &
\multicolumn{1}{c|}{\multirow{2}{*}{Type \Romannum{1}$^\ddagger$}} &   %$C^{1}$ Continuity
\multicolumn{1}{c|}{\multirow{2}{*}{Type \Romannum{2}$^\star$}} &   %Smoothness
\multicolumn{1}{c}{\multirow{2}{*}{Type \Romannum{3}$^\ast$}} \\ %Small Reality Gap
%\hline
\cline{3-10}
\multicolumn{2}{c|}{}  & 

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

% \multicolumn{1}{c|}{Mean} &  %Mean Error
% \multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{} &   %$C^{1}$ Continuity
\multicolumn{1}{c|}{} &   %Smoothness
\multicolumn{1}{c}{} \\

\hline\hline

%\color{blue}\ding{51} & \color{red}\ding{55}
\multicolumn{1}{c|}{\multirow{4}{*}{Naive Field Network}}  & 
\multicolumn{1}{c|}{(A)Recon.+ReLU}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c}{NA}  \\
\cline{2-13}

\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(B)Recon.+Lip.}  & 
\multicolumn{1}{c|}{2.53}  & 
\multicolumn{1}{c|}{11.86}  & 

\multicolumn{1}{c|}{4.32}  & 
\multicolumn{1}{c|}{24.36}  & 

\multicolumn{1}{c|}{3.01}  & 
\multicolumn{1}{c|}{21.93}  & 

\multicolumn{1}{c|}{3.61}  & 
\multicolumn{1}{c|}{32.79}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}   \\
\cline{2-13}


\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(C)Recon.+Siren}  & 
\multicolumn{1}{c|}{\color{blue}2.14}  & 
\multicolumn{1}{c|}{\color{blue}9.33}  & 

\multicolumn{1}{c|}{4.97}  & 
\multicolumn{1}{c|}{24.67}  & 

\multicolumn{1}{c|}{4.02}  & 
\multicolumn{1}{c|}{15.88}  & 

\multicolumn{1}{c|}{4.25}  & 
\multicolumn{1}{c|}{17.99}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}  \\
\cline{2-13} 

\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(D)Recon.+RBF}  & 
\multicolumn{1}{c|}{2.15}  & 
\multicolumn{1}{c|}{10.26}  & 

\multicolumn{1}{c|}{7.09}  & 
\multicolumn{1}{c|}{24.80}  & 

\multicolumn{1}{c|}{3.96}  & 
\multicolumn{1}{c|}{15.32}  & 

\multicolumn{1}{c|}{3.75}  & 
\multicolumn{1}{c|}{19.65}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}  \\


\hline \hline   %segmentation line between naive filed & rbf field
\multicolumn{1}{c|}{RBF Field Network}  & 
\multicolumn{1}{c|}{(E)}  & 
\multicolumn{1}{c|}{2.21}  & 
\multicolumn{1}{c|}{11.63}  & 

\multicolumn{1}{c|}{\color{blue}4.13}  & 
\multicolumn{1}{c|}{\color{blue}18.70}  & 

\multicolumn{1}{c|}{\color{blue}2.96}  & 
\multicolumn{1}{c|}{\color{blue}14.53}  & 

\multicolumn{1}{c|}{\color{blue}3.57}  & 
\multicolumn{1}{c|}{\color{blue}16.26}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{blue}\ding{51}}  \\
\hline\hline
\end{tabular}
\begin{flushleft}\footnotesize
$^\ddagger$ $C^1$ Continuity: measure whether the shape gradient is continuous on the surface.\\
$^\star$ Local Shape Smoothness: measure whether the local shape is changing dramatically.\\
$^\ast$ Small Reality Gap: measure the ability of the specific Sim2Real transfer to reduce error.\\
$^\dagger$ Case I: Apply actuation I to deform the prototype.
Mean and Max.: the mean and the maximum error of the calibrated model to the scanned one.\\
\end{flushleft}


%vertical space
\vspace*{2\floatsep}

%%%%%%%%%%%%%Then include Figure
\begingroup
\includegraphics[width=0.8\linewidth]{fig/figFieldPropertyComp.jpg}\\
\captionof{figure}{Experiments to test the $C^1$ continuity and smoothness of the learned field from different field learning networks: (a) (b) (c)}\label{figFieldProperty}
\endgroup

\end{table*}


















==> tex/backupFolder/texLearningBasedCtrl.tex <==
\section{Preliminary: Neural Network Based Fast Inverse Kinematics Solver}

\subsection{Problem Formulation}
The soft robotic mannequin is a actively controllable surface type soft robot with its surface denoted by  $\mathcal{S}$ can be deformed by regulating the pressures of each air chamber (denoted by $\{ \mathbf{a}_i \}$). We also have target surface shape of human body  $\mathcal{T}$ to be approximated.

Therefore, the whole control problem can be formulated as an optimization problem by minimizing two surface shape differences (The deformed shape of the mannequin $\mathcal{S}$ and the target shape of human body  $\mathcal{T}$). In the optimization problem, it is worthy mentioning that the biggest difference of our surface type control problem with the soft robot manipulator control is that our surface-surface approximation problem is much more challenging with nearly infinite DoFs and will definitely involve pose estimation ($\mathbf{R},\mathbf{t}$) during optimization steps. As a result, it is a highly non-linear problem with its objective (called \textbf{Shape Approximation Loss}) written as:

\begin{equation}\label{eqPoseEstimation}
\small
D(\mathcal{T}(\mathbf{R},\mathbf{t}),\mathcal{S}(\mathbf{a})) = \sum_{j=1}^{n}  \left\| \hat{\mathbf{p}}_j - \left(\mathbf{R} \mathbf{c}^{\mathcal{T}^*}_j + \mathbf{t} \right) \right\|^2
\end{equation}

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figLearningBasedCtrl.jpg}\\
\vspace{-2pt}
\caption{Learning-based Control for Soft Robotic Mannequin: we boost our previous gradient-based shape approximation optimizer by the neural deformation model with Sim2Real transfer (to provide analytical gradient) and initial guess network (to provide reasonable initial actuation parameters). 
}\label{figLearningCtrl}
\end{figure}


In our previous work \cite{Tian2022SoRoMannequin}, we proposed a gradient-based shape approximation optimizer with a gradient (with respect to actuation $\mathbf{a}$) calculated from hardware numerical differentiation, which means we will manually operate each actuator and record the system states, resulting in a time-consuming gradient evaluation process. What's worse, with the number of actuators increasing, the time used to calculate the gradient is increasing tremendously. 

\subsection{Fast Inverse Kinematics Solver by Forward Kinematics Neural Network}
To achieve more accurate and efficient optimization, we propose a learning-based control framework (the pipeline is shown in Fig.~\ref{figLearningCtrl} and the algorithm is listed in Alg.~\ref{algInverseKinematic}) with the gradient from differentiating the neural deformation model with Sim2Real transfer (Model detail are written in Sec.\ref{secNeuralDefModel} and the gradient computation can be found in Appendix.~\ref{Appendix:GradCompNerualDef}). With this neural deformation trained in hand, we could evaluate this analytical gradient instead of the finite difference one in the actuator space. After running the iterations in the optimizer, we could apply the optimal actuation parameters on the physical setup.

To further accelerate the optimization efficiency, an initial guess network with the convolutional neural network (CNN) has been proposed. 
\textbf{Here, we need to provide the efficiency evidence of the solver.}


\subsection{Initial Guess Network}

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figInitialGuessNN.jpg}\\
\vspace{-2pt}
\caption{Initial Guess Network for our optimizer:
}\label{figInitialGuessNN}
\end{figure}

In nonlinear optimization, the quality of the initial guess is quite important, resulting to fast convergence of the system. To further accelerate the efficiency of our solver, we modified AlexNet \cite{NIPS2012AlexNet} to take depth images (front and back) of the target model as input data to generate an initial guess for the actuation class (x in our implementation) as shown in Fig.~\ref{figInitialGuessNN}. The dataset is generated by using our learning based control method to determine optimal actuation for different target models from CAESAR dataset \cite{CAESAR2002}. Then, the optimal actuation parameters are converted into the corresponding optimal actuation class.

After training, several experiments are conducted to verify the efficiency of our network. We first select three models in the test set and another three models from different databases other than CAESAR. In experiments, our initial guess network could help reduce the steps before convergence in Fig.\ref{figInitialGuessResult}(a-c). What's more, it could also generalize to different dataset and achieve promising results in in Fig.\ref{figInitialGuessResult}(d-e). Even if in in Fig.\ref{figInitialGuessResult}(f), the target model is relatively slim, our solver achieve slightly slower convergence speed.


\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figInitialGuess.jpg}\\
\vspace{-2pt}
\caption{The effectiveness of our initial guess network: (a-e) for most cases, the network can provide reasonable initial actuation parameters for the shape approximation task, however, for some cases with slim shape (f), our initial guess network could provide similar or slightly slower convergence speed.
}\label{figInitialGuessResult}
\end{figure}






\begin{algorithm}[h]
\caption{DeepSurfIK}%DeepSurfIK
\label{algInverseKinematic}
\LinesNumbered

\KwIn{The target shape $\mathcal{T}$, the initial actuation $\mathbf{a}_0$, the initial transformation matrix $T_{0}$, relative objective function value decreasing threshold $\lambda$ and the maximally allowed iterations $i_{max}$.}

\KwOut{The optimized actuation $\mathbf{a}_{opt}$, the pose of $\mathcal{T}_{opt}$ as $(\mathbf{R}_{opt},{t}_{opt})$ and the resultant shape $\mathcal{S}_{opt}$.} 

Calculate the initial guess of the actuation parameters from the $\bold{Initial}$ $\bold{Guess}$ $\bold{Network}$ to be $\mathbf{a_0}$;

Set $i = 0$ and apply the initial actuation vector $\mathbf{a_0}$;

Evaluate the objective function $\mathcal{O}_0 =\mathcal{O}(\mathbf{a}_{0})$; 

Initialize objective function relative decreasing percentage $\mathcal{D}_0 = 1.0$;



\While{$i<i_{max}$}
{
    \tcc{Provide new transformation matrix so that objective function can continue to decrease}
    ICP-based pose estimation to get $T_{i}$ that is applied on $\mathcal{T}$ to better align with $\mathcal{S}_{i}$;

    \tcc{Gradient-based iteration with transformation fixed}
    \While{$\mathcal{D}_{i} > \lambda$ and $i<i_{max}$}
    {
    
    Compute the gradient of $\mathcal{O}(\mathbf{a}_{i})$ as $\nabla \mathcal{O}$ by differentiating neural deformation model;
    
    Set the step size $\Delta h=1.0$;
    
    Set $\mathcal{O}_{origin} = \mathcal{O}_{i}$
    
    \tcc{Soft line-search}
    
    \tcc{Step 1: Shrinking}
    
    
    \Repeat{$\mathcal{O}_{shrink} < \mathcal{O}_{origin}$}
    {
        $\mathcal{O}_{shrink} = \mathcal{O}(\mathbf{a}_{i} + \Delta h \nabla \mathcal{O})$;
        
        $\Delta h = \tau * \Delta h$;
    
    }
    $\mathcal{O}_{opt} = \mathcal{O}_{shrink}$;
    
    
    \tcc{Step 2: Expanding}
    Set $h= \Delta h$;
    
    \Repeat{$\mathcal{O}_{expand} > \mathcal{O}_{opt}$}
    {
    
    Compute and update $\mathcal{O}_{expand}=\mathcal{O}(\mathbf{a}_{i} + (h + \Delta h)\nabla \mathcal{O})$;
    
    \If{$\mathcal{O}_{expand} \leq \mathcal{O}_{opt}$}
    {
    Set $\mathcal{O}_{opt} = \mathcal{O}_{expand}$ and $h = h + \Delta h$;
    }
    
    }
    
    
    \tcc{Best $h$ has been found}
    
    Set $\mathbf{a}_{i+1} = \mathbf{a}_{i} + h \nabla \mathcal{O}$ and $i=i+1$;

    \tcc{Ready to get into next iteration}
    Evaluate the objective function $\mathcal{O}_i = \mathcal{O}(\mathbf{a}_{i})$; 

    Evaluate the objective function relative decreasing percentage as: $\mathcal{D}_{i} =\frac{\abs{\mathcal{O}_{i}-\mathcal{O}_{i-1}}}{\abs{\mathcal{O}_{i}}}$;

    
    
    }
}
\KwRet{$\mathbf{a}_{opt}$};
%\label{bla}

\end{algorithm}



% % \mathbf{return}
% $Return$
%$\mathcal{C}$;

==> tex/backupFolder/texSim2Real.tex <==
\section{Robust Sim2Real Transfer Learning}\label{secNeuralDefModel}

In robotics, learning the deformation pattern of deformable objects in simulation can be faster, safer and more informative than real physical experiments \cite{rss2020Sim2Real}. At the same time, there is no doubt that the reality gap will always remain no matter what level of advanced simulation tools are utilized\cite{rss2020Sim2Real}, which indicates the necessary step of Sim2Real transfer to bridge the gap.

In this section, we will introduce our neural deformation model boosted by Radial-basis-function (RBF) Sim2Real Transfer for the free-form surface morphing which comes with nearly indefinite Degree-of-Freedoms (DoFs) on the soft robotic mannequin, which can achieve efficient and accurate deformation pattern capturing. There exist two challenges during Sim2Real transfer:
\begin{itemize}
    \item Sparse marker dataset to calibrate surface (large DoFs) morphing in sequence (time domain).
    \item Unavoidable markers missing problem.
\end{itemize}

Considering these challenges, we leverage the power of the network and RBF to establish the pipeline. We will first introduce the learning in the simulation platform, then goes with Sim2Real transfer later.



\subsection{Simulation Forward Kinematics Learning}

\begin{figure}[t] 
\centering
\includegraphics[width=0.95\linewidth]{fig/figDataPreparation.jpg}\\
\vspace{-2pt}
\caption{Simulation Forward Kinematics Learning Dataset Preparation: (a) Our soft robotic mannequin simulator can produce chamber deformation. (b) The outer membrane can be deformed by collision detection and response with inner chambers. (c) The simulated outer membrane will be parameterized \cite{Liu2008localGlobalMeshPara}. (d) the control points\cite{BsplinesurfacesConstruction} will be further extracted to be used in the learning framework.
}\label{figDataPreparation}
\end{figure}

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figSimRepComp.jpg}\\
\vspace{-2pt}
\caption{Ablation Study of Different Surrogate Model Representation: (a) Our simulation FK network comprises of multilayer perceptron (MLP), which is used to learn the mapping between actuation parameters and surface deformation. The trained network performance on test set is drawn in (b) where we compare the point-to-mesh maximum and average distance error. The results clearly show the strongest ability of delta control point representation to approximate the simulation results.
}\label{figSimRepComp}
\end{figure}

In order to establish a surrogate model in the virtual platform to replace the time-consuming deformation simulation and provide fast and accurate gradient computation, we first carefully conduct the soft mannequin deformation simulation and extract the deformed outer membrane. After that, the extracted outer membrane will be parameterized\cite{Liu2008localGlobalMeshPara} to parametric domains. With this in hand, the B-Spline surface \cite{BsplinesurfacesConstruction} fitting is deployed to calculate the control points, which can be treated as a low-dimensional representation of the surface (as shown in Fig. \ref{figDataPreparation}). 


Note that, instead of directly learning the relationship between actuation parameters and vertex positions (which will cause larger errors in Fig.\ref{figSimRepComp}), the delta control points( current control points subtracting the locations of undeformed control points) are used as an effective way to represent the surface deformation. That is, we learn the control point offsets by the network. In our ablation study in Fig.\ref{figSimRepComp}, it is clear that the average point-to-mesh average distance error is reduced from 4.99 mm and 1.74 mm to 0.75 mm (reduce 84.97
\%). The average point-to-mesh maximum error is decreased from 21.11 mm and 15.01 mm to 4.47mm (reduce 78.83 \%). In short, the delta control points will be used throughout the paper as simulation representation.

\subsection{Field Sim2Real Transfer with Limited and Incomplete Data}

According to the panel discussion in \cite{rss2020Sim2Real}, it is important to have Sim2Real for the transfer of learning the reality gap. 
The first choice is to naturally learn the surface shape to surface shape mapping. However, there are several limitations exist in this architecture:

\begin{itemize}
    \item Requiring dense ground-truth information (r.g., scanning mesh, point cloud from RGB-D camera, or dense marker array) and the correct correspondence among captured sequences for the training. 
    \item Sophisticated data collection process to ensure captured range, clear boundary, and marker completeness (if we choose dense marker array).
    \item Tedious post-processing steps are involved, including data cleaning, parameterization and so on.
\end{itemize}

Especially if we use scanner to capture the ground-truth info, it is impractical to acquire the whole scanned mesh with perfect topology (e.g., has clear sharp features, no small holes, and no intersection), which is important to be processed to be B-Spline control points. For RGB-D devices that come with point clouds, it is hard to ensure the captured range is the same as the simulation one. Furthermore, the parameterization of point clouds is hard to consistent throughout the whole capture sequence (with different shapes). If we choose a dense marker set to provide a label, it will easily bring the problem of marker missing, which can not be solved by this architecture.

If we insist on having this strict requirement, it would highly increase the data collection and processing workload, which somehow conflicts with the real purpose of Sim2Real: lightweight data collection.

To solve these problems altogether, we reformulate the sim2Real transfer problem as the implicit field learning problem and propose an implicit learning framework as shown in Fig.\ref{figFieldPipeline} (b).

The network structure takes only one query point (on the simulation surface) and latent code $\mathbf{Z}$ (conditioning surface shape space) as input in Fig. (b). This allows marker missing problems. At the same time, the attached marker array is sparse (nearly 35 markers) compared to the dense surface DoFs. In this way, our field Sim2Real learning pipeline can lower the data collection burden and guarantee its generality.

To the best of our knowledge, it is the first time that a general Field Sim2Real Transfer architecture (two different types are shown in Fig. \ref{figFieldPipeline}) for free-form surface morphing is proposed. Its effectiveness has been verified in the soft robotic mannequin scenario which can be seen in Sec.\ref{}.



\begin{figure}[h] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figFieldLearning.jpg}\\
\vspace{-2pt}
\caption{Two different types of field Sim2Real Transfer Network: (a) Naive Field Sim2Real Transfer. The input of the Sim2Real Network contains two parts: 1) simulation position on the simulation surface and 2) encoded latent code Z which further compresses the information of surface to low-dimension space. For each input simulated surface point, our NN will output the calibrated point on the real surface. Another Network is (b) RBF Field Sim2Real Transfer. In this network, we first predict the RBF coefficients, and by interpolating with simulation anchor points, we can output the calibrated surface by querying every point on the simulation surface.
}\label{figFieldPipeline}
\end{figure}

To prove the superiority of our field learning Sim2Real architecture (Fig. \ref{figFieldPipeline})(b)), we have proposed a naive field Sim2Real pipeline (Fig. \ref{figFieldPipeline})(a)) and done some ablation studies.


\subsubsection{Naive Field Sim2Real Network}
\label{secNaiveField}
The naive field learning pipeline (in Fig.\ref{figFieldPipeline}(a)) directly predicts the calibrated point $\mathbf{\hat{q}}_{sj}$ by feeding the query point $\mathbf{q}_{sj}$ and encoded $\mathbf{Z}$ vector into the network. In this section, four baselines using different activation functions and loss functions are implemented to test the Sim2Real error. 

The first baseline is finished by only imposing reconstruction loss, and the trained field can be visualized by feeding simulation vertices into the trained network and constructing the calibrated mesh as shown in Fig.~\ref{figReconOnly}, which shows the field is non-smooth across the whole domain.

\begin{figure}[h] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figReconLossOnly.jpg}\\
\vspace{-2pt}
\caption{Calibrated Surface by Naive Field Sim2Real Network with Recon. Loss only.
}\label{figReconOnly}
\end{figure}



The second baseline is adding one extra Lipschitz regularization term \cite{liu2022lipLoss} into total loss in the training process. In the
Fig.~\ref{figReconLip}, we have applied different actuation parameters on the real physical setup, simulation platform, and naive field Sim2Real Network with Recon. and Lip. Loss. In Fig.~\ref{figReconLip}(a) where all actuation is set to zero, the simulation result has large errors around the belly region considering our double-layer design brought manufacturing imperfection (increase the membrane thickness here). It is exciting to observe that our Sim2Real network can adjust this error with the maximum error, average error, and standard deviation reduced by $18.5\%$, $20.2\%$, and $23.1\%$ respectively. In Fig.~\ref{figReconLip}(b), with maximum actuation applied on setup, it is further observed that our naive field Sim2Real network can achieve much better accuracy with $27.1\%$, $51.4\%$, and $36.5\%$ reduction on the maximum error, average error, and standard deviation.

However, this naive field NN (with Recon. Loss and Lip. Loss) can not faithfully preserve local shape details as shown in Fig.~\ref{figReconLip}(a), especially in the zoom-in areas. What's more, the laplacian (\cite{Sorkine2005Laplacian}) gradient norm is drawn in colormap and histogram to validate this conclusion.
\begin{figure}[h] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figReconLipExp.jpg}\\
\vspace{-2pt}
\caption{Calibrated Surface by Naive Field Sim2Real Network with Recon. Loss and Lip. Loss: (a), (b) \& (c): the Sim2Real network can successfully reduce simulation non-linearity and manufacturing imperfection.
}\label{figReconLip}
\end{figure}

\begin{figure}[h] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figLipSmoothVariation.jpg}\\
\vspace{-2pt}
\caption{Calibrated Surface by Naive Field Sim2Real Network with Recon. Loss and Lip. Loss: (a) it cannot preserve local shape property, the local shape detail variation is changing dramatically as shown in (b) where a larger value indicates the worsened shape preserving. 
}\label{figLipSmoothVar}
\end{figure}



The third baseline is the naive field Sim2Real NN with Recon. Loss and Siren activation function \cite{sitzmann2020implicit}. In Fig.~\ref{figReconSiren}(d), the siren activation function could achieve better detail-preserving than NN with Lip. Loss. However, its Sim2Real error is still undesirable when the deformable mannequin is with large inflation shape: around $14.8\%$ and $17.6\%$ percent increase on the average error compared to results with NN of Lip. Loss.

\begin{figure}[h] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figReconSirenExp.jpg}\\
\vspace{-2pt}
\caption{Calibrated Surface by Naive Field Sim2Real Network with Recon. Loss and Siren Activation: (d): Siren activation can improve the local shape preserving but can not improve Sim2Real error to the level of NN with Lip. Loss (a-c).
}\label{figReconSiren}
\end{figure}


The final baseline is the naive field Sim2Real NN with RBF Layer with its parameters tuned during the training. After training, we visualize its sim2real error in Fig.~\ref{figReconRBFNaive}(a-c), the sim2real error is increased tremendously, especially the average error for Fig.~\ref{figReconRBFNaive}(b) and (c) with 7.09 mm ($63.8\%$) and 3.98 mm ($27.0\%$). The property comparison is listed in Table. ~\ref{tab:naiveFieldComparison}.

\begin{figure}[h] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figReconRBFLayerExp.jpg}\\
\vspace{-2pt}
\caption{Calibrated Surface by Naive Field Sim2Real Network with Recon. Loss and RBF Layer: (d): RBF layer can improve the local shape preserving but can not improve Sim2Real error to the level of NN with Lip. Loss (a-c).
}\label{figReconRBFNaive}
\end{figure}




\begin{table}[h] \footnotesize%\tiny %scriptsize
%\footnotesize
\centering

% \jun{Should modify to coherent with three categories definition}
\begin{tabular}{cc|c|c|c}         %adjust column number 
\hline \hline                       %horizontal line
\specialrule{0em}{2pt}{1pt}         %vertical space
\multicolumn{2}{c|}{\multirow{2}{*}{\textit{}~}}  & \multicolumn{3}{c}{Property} \\ %column arrangement
\specialrule{0em}{1pt}{2pt}         %vertical space
\cline{3-5}                        %segementation line
\specialrule{0em}{2pt}{1pt}         %vertical space

% \multicolumn{2}{c|}{\multirow{2}{*}{\textit{}~}}  
\multicolumn{2}{c|}{Network Type}  
% & \multicolumn{1}{c|}{Shape $C^1$ Continuity} & \multicolumn{1}{c|}{Local Shape Preserving}  & \multicolumn{1}{c}{Small Sim2Real Error} 
& \multicolumn{1}{c|}{Type A$^\dagger$} & \multicolumn{1}{c|}{Type B$^\star$}  & \multicolumn{1}{c}{Type C$^\ddagger$} 
\\ 

%Recon. Only: \ding{55} is wrong, \ding{51} is right
\specialrule{0em}{1pt}{2pt}
\hline \specialrule{0em}{1pt}{2pt}
\multicolumn{2}{c|}{Naive Field (Recon.)} & \color{red}\ding{55} & \color{red}\ding{55} & \color{red}\ding{55}\\

\specialrule{0em}{1pt}{2pt}
\hline \specialrule{0em}{1pt}{2pt}
\multicolumn{2}{c|}{Naive Field (Recon. + Lip.)} & \color{blue}\ding{51} & \color{red}\ding{55} & \color{blue}\ding{51}\\

\specialrule{0em}{1pt}{2pt}
\hline \specialrule{0em}{1pt}{2pt}
\multicolumn{2}{c|}{Naive Field (Recon. + Siren)} & \color{blue}\ding{51} & \color{blue}\ding{51} & \color{red}\ding{55}\\

\specialrule{0em}{1pt}{2pt}
\hline \specialrule{0em}{1pt}{2pt}
\multicolumn{2}{c|}{Naive Field (Recon. + RBF Layer)
} & \color{blue}\ding{51} & \color{blue}\ding{51} & \color{red}\ding{55}\\

\specialrule{0em}{1pt}{2pt}
\hline \specialrule{0em}{1pt}{2pt}
\multicolumn{2}{c|}{RBF Field Sim2Real (Ours)
} & \color{blue}\ding{51} & \color{blue}\ding{51} & \color{blue}\ding{51}\\

\specialrule{0em}{0pt}{2pt} \hline\hline
\end{tabular}

\begin{flushleft}\scriptsize
$^\dagger$ $C^1$ Continuity: measure whether shape is continuous for the gradient of the surface.\\
$^\star$ Local Shape Preserving: measure whether local shape is changing dramatically.\\
$^\ddagger$ Small Sim2Real Error: measure the Sim2Real transfer ability to reduce error.\\
\end{flushleft}

\caption{Comparison of Different Field Learning Network Performance.}\label{tab:naiveFieldComparison}
\vspace{-10pt}
\end{table}




\subsubsection{RBF Field Sim2Real Network}
The field learning network in Sec.~\ref{secNaiveField} directly learns the shape-to-shape relationship with different activation and loss functions. However, they are not capable of  simultaneously satisfying the requirements of $C^{1}$ continuity, local shape preserving, and small Sim2Real error. 

Considering this, we propose a RBF Field Sim2Real Network (see Fig.~\ref{figFieldPipeline})(b) which gives up directly finding the field mapping between the simulation field and the real field only via MLP. Instead, it establishes the relation from the simulation shape space to the intermediate function space (RBF coefficients\cite{Charlie2007RBFVolPara}). Then, with the predicted function space values, the RBF functions will constitute the transferred shape by interpolating the whole real field by traveling the whole simulation surface using the equation below: 


\begin{equation}
\label{equRBF}
    \mathbf{\hat{q}}_{sj} = \mathbf{a_{0}} + \mathbf{A}\mathbf{\hat{q}}_{sj} +
   \sum_{i=1}^{N} \mathbf{b}_i g(\mathopen| \mathbf{q}_{sj} - \mathbf{q}_{i} \mathclose|)
\end{equation}

in Eq.\ref{equRBF}, rbf coefficients are $\mathbf{a}_0$, $\mathbf{a}_1$, $\mathbf{a}_2$, $\mathbf{a}_3$ and $\mathbf{b}_i$ as column vector. $\mathbf{A}$ matrix can be further written as:

$$\mathbf{A}=
\bigg[\begin{array}{c|c|c}
\mathbf{a}_1 &\mathbf{a}_2 &\mathbf{a}_3
\end{array}\bigg]
$$

In eq.\ref{equRBF}, we can think $\mathbf{\hat{q}}_{sj}$ is represented from a set of basis vectors ($\mathbf{a}_i$ and $\mathbf{b}_i$) with their weighting as radial basis function $g(\mathopen| \mathbf{q}_{sj} - \mathbf{q}_{i} \mathclose|)$ where $g(*)$  is chosen to be Gaussian $\phi(r) = e^{-cr^2}$  (\cite{Carr2001RBF}).
We don't learn the shape-to-shape relationship directly, What we learn is different sets of function bases that correspond to the different input surfaces.

As a result, the learned result is quite promising which results in more smooth and natural shapes considering this representation guarantees at least $C^2$ continuity. At the same time, this representation is based on the anchor points on the simulation shape, which serve as physical prior during learning, enabling the RBF field learning to accurately capture the shape offset from the simulation field to the real field. At the same time, this field learning architecture tolerates the markers missing problem.

\begin{figure}[h] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figRBFSim2Real.jpg}\\
\vspace{-2pt}
\caption{Calibrated Surface by RBF Field Sim2Real Network: (d): this network can better achieve the local shape preserving and also be able to reduce Sim2Real error compared to the best performed naive Field Sim2Real with Recon. Loss and Lip. Loss.
}\label{figReconRBFSim2Real}
\end{figure}

In Fig.~\ref{figReconRBFSim2Real}, the proposed RBF Field Sim2Real network can achieve more accurate and stable calibrated results across all shapes. Especially when it is the fat shapes, our proposed pipeline reduces the maximum error by $23.2\%$, $33.7\%$ and $50.4\%$ respectively in Fig.~\ref{figReconRBFSim2Real} (a-c). Furthermore, it can achieve local shape preserving as shown in Fig.~\ref{figReconRBFSim2Real} (d) with an average value reduced by $36.4\%$ and a maximum value reduced by $45.0\%$.



==> tex/secImplementation.tex <==
\section{Implementation Details \& Experimental Results}\label{secImplementation}

\subsection{Parameterization}
\label{secPara}
 Parameterization is a technique used to assign each vertex of the mesh a uv value \cite{Sheffer2006Para} so that the mesh can be flattened to a simple and regular domain (e.g., planar regions). This technique can be used in various applications, such as texture mapping, detail transfer, and surface fitting. In our case, parameterization is used to assist the surface fitting to reduce the dimensionality of the free-form surface by extracting the surface control points as descriptors to feed into the neural network for better training (see Sec.\ref{secNeuralDefModel}).

 The right corner of Fig.\ref{figDataPreparation} illustrates the whole procedures for soft free-form surface parameterization that is used in our soft mannequin setup. The first step is to cut the mesh by the polyline based on the geodesic distance \cite{Vitaly2005FastGeodesicDis} between two endpoints (from top and bot circle respectively). As shown in Fig.\ref{figDataPreparation}, the cutting polyline is shown as the intersection between red triangles and blue triangles with the cut point as a green dot. Note that, after cutting, there are two points on the same cutting point to split the surface into homeomorphic to square. 

 %Furthermore, the cut mesh would have two boundary curves on the back where the cut happened as indicated by red and blue arrows. 
Then, an efficient ARAP parameterization method \cite{Liu2008localGlobalMeshPara} would be applied to generate the UV pairs for each vertex of the cut mesh, which will be visualized by the checkerboard in Fig.\ref{figDataPreparation}.
%  \begin{figure}[h] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figParameterization.jpg}\\
% \vspace{-2pt}
% \caption{Parameterization for the outer membrane of the soft robotic mannequin: a) The outer membrane will be cut (intersection line between red and blue region) to make it topologically equivalent to a square. b) The cut mesh has two boundary curves at the back with its direction drawn in red and blue. c) The cut mesh will be processed by ARAP mesh parameterization method~\cite{Liu2008localGlobalMeshPara}. 
% }\label{figPara}
% \end{figure}


% \subsection{Initial Guess Network}
% \label{secInitGuessNN}

% \begin{figure}[h] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figInitialGuessNN.jpg}\\
% \vspace{-2pt}
% \caption{Initial Guess Network for our optimizer:
% }\label{figInitialGuessNN}
% \end{figure}


% In nonlinear optimization, the quality of the initial guess is quite important, resulting to fast convergence of the system. To further accelerate the efficiency of our solver, we modified AlexNet \cite{NIPS2012AlexNet} to take depth images (front and back) of the target model as input data to generate an initial guess for the actuation class (eight in our implementation) as shown in Fig.~\ref{figInitialGuessNN}. The dataset is generated by using our Fast IK solver to determine optimal actuation for different target models from CAESAR dataset \cite{CAESAR2002}. Then, the optimal actuation parameters are converted into the corresponding optimal actuation class.

% After training, several experiments are conducted to verify the efficiency of our network. We first select three models in the test set and another three models from different databases other than CAESAR. In experiments, our initial guess network could help reduce the steps before convergence in Fig.\ref{figInitialGuessResult}(a-c). What's more, it could also generalize to different datasets and achieve promising results in in Fig.\ref{figInitialGuessResult}(d-e). Even if in Fig.\ref{figInitialGuessResult}(f), the target model is relatively slim, our solver achieves a slightly slower convergence speed.



% \begin{figure}[h] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figInitialGuess.jpg}\\
% \vspace{-2pt}
% \caption{The effectiveness of our initial guess network: (a-e) For most cases, the network can provide reasonable initial actuation parameters for the shape approximation task, however, for some cases with slim shape (f), our initial guess network could provide similar or slightly slower convergence speed.
% }\label{figInitialGuessResult}
% \end{figure}



\subsection{Hardware System}
In this section, we will introduce the hardware system, which consists of a soft robotic mannequin, a closed-loop pressure control system, and two vision devices.



\subsubsection{Design and Fabrication of Soft Robotic Mannequin}
Our soft robotic mannequin has a three-layer design with an inner soft chamber layer (which can be deformed by pressurized air) attached to base solid chambers, a middle soft chamber layer attached on top of the inner layer (which can also be inflated), and a top membrane layer (passively morphed) covering the base layers to form the overall smooth shape. By actuating the inner and middle layers by pumping air inside the chamber \cite{Tian2022SoRoMannequin} to different pressures, the soft robotic mannequin will be deformed (Fig.\ref{figTeaser}) into different shapes. 

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figFab.jpg}\\
\vspace{-2pt}
\caption{Fabrication Steps of the soft robotic mannequin: (a-b) We design, fabricate, and seal a sequence of molds to create a tightly enclosed space. Within this space, liquid silicone is injected, and after a few hours, it transforms into a cohesive soft layer (c-d). For the outer membrane, three molds (one inner mold and two outer molds) are created to be injected with silicone. After consolidation, it will be attached to the top of the mannequin to form the overall shape. 
}\label{figFab}
\end{figure}

The fabrication steps are illustrated in Fig.\ref{figFab}. The basic idea of the fabrication is to cast silicone into the spare space enclosed by our carefully designed molds. For the inner layer with 14 chambers, we designed 8 molds (shown in Fig.\ref{figFab}(a)), which will form the empty space before silicone casting as shown in Fig.\ref{figFab}(b). By injecting the liquid silicone (Dragon Skin 20~\cite{DS20}) from the lowest point to the highest point, a group of soft chambers with 2 mm thickness will be fabricated after 4 hours of curing as shown in Fig.\ref{figFab}(c). For the middle soft layer, we seal the two soft membranes to form the inflatable bag and attach it to the first layer as shown in Fig.\ref{figFab}(d).

For the top layer of the outer membrane, we designed one inner mold and two outer molds, which will form the space (Fig.\ref{figFab}(f)) to be cast silicone Ecoflex 00-30 \cite{EC30} inside. Finally, after acquiring the consolidated membrane, we have attached it to the top of the base and middle layers to form the mannequin with a soft and deformable free-form surface (Fig.\ref{figFab}(h)). For more details for the casting, please refer to \cite{Tian2022SoRoMannequin}.


\subsubsection{Actuation and Vision System}
During experiments, to achieve controlled pneumatic actuation, we have built an open-source pneumatic platform called OpenPneu (\cite{tian2023openpneu}), to provide multi-channel controlled pressure. It can be easily operated by sending target pressures through serial communication. 

To get the ground-truth information for our RBF field Sim2Real transfer network and FastIK solver, two vision devices are utilized as shown in Fig.\ref{figTeaser}, including Vicon motion capture system\cite{Vicon} (which will be used to collect marker locations on the deformable mannequin, which is processed to be dataset for Sim2Real network training) and Artec Eva Lite scanner, a structured-light-based scanner\cite{Scanner} to collect scanned ground-truth mesh of the surface to verify the Sim2Real and FastIK results. 


==> tex/secIntroduction.tex <==
\section{Introduction}
\label{secIntro}

\Guoxin{Rewrite on Jan 03, 2024 - new version Jan 25}

\Tian{careless use of self-citations can easily violate the requirements for double blind reviewing and this will result in papers being desk rejected -- RSS}

\IEEEPARstart{R}{obotics} deformable surfaces have demonstrated the ability to dynamically adapt their shape and structure in response to programmed commands or environmental stimuli. Over the past decades, various prototypes have been developed across diverse fields, including \textit{human-computer interaction} (HCI) as interactive surfaces~\cite{Stanley2015CtrlSurf,Je2021ElevateAW,inForm2013UIST}, soft robotics~\cite{Bryan2019SoRoInterface}, and medical prosthetics for medical phantoms, providing customized solutions for CRP training as detailed in~\cite{inFORCE2019TEI}. Another particularly notable application of robotics deformable free-form surfaces is in the garment industry. Tian~\textit{et al.}~\cite{Tian2022SoRoMannequin} developed a pneumatic-driven soft robotics mannequin capable of deforming and mimicking human body shapes from the front side. With four pneumatic-driven chambers and an outer skin, it presents continuous shape change with a smooth surface representation, therefore not only enhancing the fit and personalization of garments but also contributing significantly to reducing waste and return rates in the industry, issues that are highlighted in the textile industry report~\cite{textileReport2017}. In this work, we present the \textit{SoRo-Mannequin} II, a free-form surface system which substantially improves the design and control ability over the previous version.


\begin{figure*}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figTeaser.jpg}\\
\caption{ (a) We propose a novel soft robot mannequin design that allows free-form shape to deform to matching human shape with both front and back view. (b) To enable fast IK computing control for shape matching, we propose a robust sim-to-real learning-based pipeline to not only provide end-to-end evaluation on the gradient between shape and actuation parameters but also narrow the Sim2Real gap. This network tackles the challenge that (c) data collection from physical setup are generally slow and unrobust.\Tian{Need to select models (with RGB from dataset)}}
\label{figTeaser}
\end{figure*}

%% Guoxin: Briefly mention the advantage of new prototype.

As illustrated in the middle of Fig.~\ref{figTeaser}(a), the \textit{SoRo-Mannequin} II is outfitted with fifteen controllable chambers with nine independent DoFs. These chambers, pneumatically driven by air pressure, can morph to approximate a diverse range of human body shapes ${\mathcal{S}^T}$, 
featuring substantial variations on both the front and back. This represents a significant advancement over our initial version, which was limited to a single side with only four DoFs. The new design incorporates considerations of human anatomy to create a chamber with freeform shape morphing ability 
%(details are discussed in Sec.xx\Tian{Will describe this in implementation details later})
, enabling the deformable surface to achieve sufficient deformation space. This design capability allows for the approximation of a wide spectrum of human body shapes ${\mathcal{S}^T}$, covering an extensive range (xx\% coverage) of human shapes in sizes 4-9 from the CAESAR Dataset\cite{CAESAR2002}.

\subsection{Challenges in IK computing for freeform surface.}

While increasing the number of chambers and the complexity of shapes significantly enhances the shape-morphing ability of the system, effectively computing the actuation parameters $\mathbf{a}$ to facilitate rapid shape morphing ($\mathcal{S}$) and approximate target shapes $\mathcal{S}^T$ is crucial for practical applications, yet it presents considerable complexity. In the \textit{SoRo-Mannequin} II setup, the forward kinematic mapping from the actuator space to the configuration space is defined as $\mathcal{A} \in \mathbb{R}^{9} \rightarrow \mathcal{S}\in\mathbb{R}^{\infty}$\Tian{18 is changed to 9 because of the independent DoFs}. The process of determining the actuation parameters for a given target shape is equivalent to computing the \textit{inverse kinematics} (IK) solution. In our previous work~\cite{Tian2022SoRoMannequin}, we introduced surface parameterization with B-spline control points to facilitate IK computation using a Jacobian-based iterative approach. However, computing the gradient of the shape function through numerical differentiation on the hardware~\cite{Tian2022SoRoMannequin,Yip2014TROHardwardGradient} can be extremely slow, primarily due to a single gradient requiring multiple time-consuming shape evaluations on the physical setup. This challenge is even worse on the newly developed full-body mannequin - since a robust yet efficient capture of the freeform shape on both sides is not available. As illustrated in Fig.~\ref{figTeaser}(b), using a 3D scanner to capture point clouds or employing a motion capture system to track high-precision marker positions can lead to stability problems, often due to non-constant scanned boundary connection, marker loss, and region occlusion.

In robot systems characterized by compliance and high Degrees-of-Freedom (DoFs) in the configuration space, learning-based methods are highly efficient in providing fast IK solutions for tasks like deformable object manipulation, continuum/soft robot control, and soft tissue manipulation. These methods typically employ data-driven approaches to fit the Forward Kinematics (FK) and can rapidly approximate the Jacobian based on the network’s gradient. We adopt this approach in our work as well, where the mapping from the actuation space to a (reduced) parameter space representing the free-form surface is applied, as depicted in $N_{sim}$ \Tian{I might need to illustrate $N_{sim}$} in Fig~\ref{figTeaser}(b). However, directly training the network with physical data is impractical due to the data generation challenges inherent in our \textit{SoRo-Mannequin} II system. Systems with compliance generally suffer from the difficulty of massive data collection in a physical setup, which has also been reported in \cite{Zhao2020Sim2RealSurvey}. An efficient alternative involves first collecting data from a physics-driven virtual platform with a trained model, then applying sim-to-real transfer learning to achieve robust physical performance~\cite{Zhao2020Sim2RealSurvey,rss2020Sim2Real}. Existing research primarily focuses on the task space of robot systems, where ground-truth data are relatively easy to obtain from vision systems (e.g., the tip position/orientation of a manipulator with no more than six DoFs from a motion capture system~\cite{Thomas2018SoRoCtrlReview}). In contrast, our work deals with the configuration space of deformable surfaces (with nearly indefinite DoFs), where data generation can be challenging and has been less explored in existing research.

\subsection{Our solution and Contribution}
In this work, we implement a robust sim-to-real transfer strategy to facilitate fast FK evaluation of the deformable surface, thereafter assist a rapid IK computation for the control of \textit{SoRo-Mannequin} II. Tackle the challenge of unrobust and sparse physical data given for sim-to-real transfer, an approach includes learning the function space for an implicit field using \textit{radial basis functions} (RBF), which forms a neuron-based representation of shape morphing in high-dimensional deformable surfaces, as depicted in Fig.~\ref{figTeaser}. The RBF function has proven effective in spatial extrapolation capabilities, capturing the shape morphing between shape data of free-form surfaces across both the comprehensive virtual space and the sparse yet incomplete physical space. This approach provides a robust sim-to-real transfer learning that fully leverages the entire physical dataset and can benefit from all the sigle vertex point as input to inflect the whole space warping function $W(\cdot)$. Combined with the FK learning network, we can offer an analytical solution for approximating the shape function's Jacobian, thus enabling fast IK computing for 3D deformable free-form surfaces. This strategy effectively bridges the commonly identified reality gap and addresses the challenges of data generation from the physical setup of the robotic deformable surface. \Guoxin{to highlight that we can obtain single-shoot direct parameters computing to fit target shape with neuron-based FK and sim-to-real assisted IK.}

We conducted tests on the newly developed \textit{SoRo-Mannequin} II setup using our proposed learning-based fast IK solver. The virtual dataset, comprising xx data points, was collected from our rapid geometry-based simulator and then integrated with a physical dataset containing xx data points. Notably, 18 out of 30 data points in the physical dataset had missing marker ground-truth data, yet we still achieved robust sim-to-real transfer results. The accuracy of the system improved, achieving a precision of xx mm (\%xx of the workspace) in shape optimization. On average, the computing time for the IK solution on the physical setup was xxs, which is sufficiently rapid for application in this setup (in comparison, the actuation time is xx).

\Guoxin{Above introduction section rewrite at 29 Dec 2023.}


The technique contributions of this work can be summarized into:
\begin{itemize}
    \item A robust Sim2Real transfer learning framework that takes sparse and even incomplete ground-truth information to bridge the reality gap with implicit field representation and Radial Basis Function (RBF) for soft surface morphing with nearly indefinite DoFs. 
    \item A fast IK solver based on neural networks that solves the surface-to-surface approximation problem with analytical gradient for the soft robotic mannequin.
     \item A robotic deformable soft mannequin system named SoRo-Mannequin II consisting of both hardware and intelligent algorithms is built to validate the robustness and accuracy of our Sim2Real pipeline and Neural network-based IK.
\end{itemize}

\begin{comment}
    
\Guoxin{Second Paragraph: In this work, we present soft robot mannequin 2 - extend to full body shape and contains 18 actuations - a number that existing method hard to realize gradient-based IK \Tian{Added}. While learning-based solution is presented in [][], (present how they work) however they are all limited in virtual space. \Tian{Maybe this comparison is not fair, I quote some common examples for learning based IK from Coros that establish differentiable FK and insert into IK solver. I also use the conclusion from RSS workshop on Sim2Real: 1) FK learning on Sim is more informative. 2) FK learning from sim only is not enough. Use these two conclusions to indicate the importance of Sim2Real}}

\Guoxin{To elimiate reality gap and enhance the effeciency of data generation, sim-to-real learning is applied. However, [Robust!!!! - why the existing method is not \textbf{robust}? with motion capture system] - teaser is need to explain what is define as unRobust.\Tian{added}}

\Guoxin{Therefore in this work we present... differentiable end-to-end sim-to-real with implicit field functions learning. -> How this can solve the aforementioned issue.}\Tian{Added}

\Guoxin{Sim-to-real module is part of the network-based solution, and we also present new soft mannequin design, fabrication, and fast IK.}\Tian{Added, I think the design and fabrication might not be the key points, but I do mention sim2Real is part of network-based IK.}

\Guoxin{Related work}\Tian{Aleady adjust to before contribution}

\Guoxin{contribution}\Tian{Added}



Currently, the utilization of free-form surface representation in the garment industry unlocks the potential for the design, optimization, and manufacturing of made-to-measure garments catering to individual preferences and body measurements~\cite{aldrich2007history}, particularly through the utilization of customized physical avatars (mannequins \cite{Alvanon}). This approach holds the promise of mitigating the significant return rates and, concurrently, addressing the substantial wastage of resources in the industry~\cite{textileReport2017}.

However, presenting only one specific free-form surface shape for each mannequin is expensive resulting in escalated costs \cite{Alvanon}. As a result, morphable free-form surface is needed to assist in tailored garment design for achieving mass customization across diverse customer profiles.

To address this challenge, a soft deformable mannequin, which can achieve active surface morphing, is proposed \cite{Tian2022SoRoMannequin}. However, the gradient-based inverse kinematics (IK) solver proposed in this paper falls short in efficiently approximating target shapes mainly from the calculating gradients from hardware differentiation\cite{Tian2022SoRoMannequin, Yip2014TROHardwardGradient}, constraining its utility for real-time fitting of diverse target models. 

In this work, we further present SoRo-Mannequin II, which has been extended to cover full body deformation with nine independent pneumatic actuators - a number that existing model-less methods hard to realize efficient inverse computation.

Usually, a common practice of a fast IK solver is to build a forward kinematics (FK) model in an end-to-end manner, and insert this FK model into the iterative IK solver \cite{bern2019trajectory, bern2020soft}. As a result, a fast and accurate neural deformation model is needed to establish the mapping between actuator space and configuration space\cite{Thomas2018SoRoCtrlReview} in an end-to-end manner. 

The neural deformation model trained from simulation data can be faster, safer, and more informative than real physical experiments \cite{rss2020Sim2Real}. Also, there is no doubt that the reality gap will always remain no matter what level of advanced simulation tools are utilized\cite{rss2020Sim2Real,Zhao2020Sim2RealSurvey}, which indicates the necessary step to transfer the robot state from simulation to reality (called "Sim2Real transfer") in FK modeling.

In previous work, the Degree-of-Freedoms (DoFs) of

Sim2Real is usually limited and each captured data frame is complete (\cite{Fang2022Sim2Real, Gomes2023Sim2RealTactile, peng2018sim}). However, in robotics, there is no prior work about sim2real for free-form surface morphing with indefinite DoFs to be described. Also, during the Sim2Real step, it is a common phenomenon that ground-truth information with large DoFs is usually incomplete for long-time capturing as shown in Fig.\ref{figTeaser}(c).


To reduce the workload of Sim2Real capturing by leveraging only a limited number and even partially missed ground-truth data, we reformulate our surface Sim2Real problem into an implicit field learning problem, combining with radial basis function, we proposed a novel and robust Sim2Real pipeline with an end-to-end analytical gradient to solve the aforementioned issues as shown in Fig.\ref{figTeaser}.

In this paper, we validate the feasibility of our Sim2Real pipeline through comprehensive experiments. We further validate the FastIK solver with Sim2Real embedded to complete the multi-target shape approximation task on our physical prototype: SoRo-Mannequin II. 


\subsection{Our Method}

In this paper, for the first time, we present the Sim2Real learning for surface morphing with indefinite DoFs. We reformulated the problem as an implicit field learning problem to address the partial data missing challenge. To further achieve accurate training, the implicit field is not directly learned. Instead, we learn the function space of RBF, which is utilized to construct the implicit field using space warping\cite{Charlie2007RBFVolPara}.

With this robust Sim2Real in hand, we further construct the Fast IK framework to achieve a multi-target shape approximation task with physical experiments validated on our soft robotic mannequin system.

The technique contributions of this work can be summarized into:
\begin{itemize}
    \item A robust Sim2Real transfer learning framework that takes sparse and even incomplete ground-truth information to bridge the reality gap with implicit field representation and Radial Basis Function (RBF) for soft surface morphing with nearly indefinite DoFs. 
    \item A fast IK solver based on neural networks that solves the surface-to-surface approximation problem with analytical gradient for the soft robotic mannequin.
     \item A robotic deformable soft mannequin system named SoRo-Mannequin II consisting of both hardware and intelligent algorithms is built to validate the robustness and accuracy of our Sim2Real pipeline and Neural network-based IK.
\end{itemize}

\end{comment}


\section{Related Work}


\begin{figure*}[h] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figDataPreparation.jpg}\\
\vspace{-2pt}
\caption{ FastIK Solver (Virtual Platform) is proposed to achieve efficient computation of optimal actuation parameters based on a given target model. It includes a neural deformation model aiming at replacing the time-consuming simulation process and post-processing steps (extract free-form surface descriptors as dimension reduction). This surrogate model provides repaid shape and analytical gradient computation, successfully supporting the efficient computation of FastIK solver.
%Simulation Forward Kinematics Learning Dataset Preparation: (a-b) Our geometry-based simulator could predict the deformation and generate the outer membrane shape (\cite{Guoxin2020TRO, Guoxin2022IROS}). (c) The membrane will be parameterized \cite{Liu2008localGlobalMeshPara} and fitted to extract the control points\cite{BSpline1974Book} as the lower dimension representation to be used in the learning framework.
\Tian{Figure and Section. \ref{secNNFastIK} rewritten   Jan 14}
}\label{figDataPreparation}
\end{figure*}


\subsection{Sim2Real Transfer}

Sim2Real Transfer has recently garnered significant attention from researchers in the field of robotics. Three Sim2Real workshops were conducted in 2019, 2020, and 2022 \cite{sim2realRSS2022WebPage}. It is widely acknowledged that training based on simulation data offers a cost-effective approach to policy learning, especially when compared to the expensive and occasionally perilous collection of physical data \cite{rss2020Sim2Real, Zhao2020Sim2RealSurvey}. However, relying solely on simulation-based training introduces inherent disparities with real-world physical scenarios \cite{Zhao2020Sim2RealSurvey}. This underscores the considerable advantage of Sim2Real transfer learning.

In the realm of rigid robots, Sim2Real learning has found application in diverse domains such as drone navigation \cite{kaufmann2020RSS}, imitation learning for locomotion skills \cite{peng2020learning}, and enhancing dexterous manipulation capabilities \cite{akkaya2019solving}.

In soft robotics, Sim2Real has been applied in design (\cite{shah2021soft, Kriegman2020Sim2RealSoRoDesign}), modeling (\cite{Dubied2022Sim2RealFEM, Zhang2022Sim2RealSoRoFish}), sensing (incorporating vision-based tactile sensors \cite{Gomes2021Sim2RealGelSight, Luu2023Sim2RealVisionTactile, Gomes2023Sim2RealTactile}) and control (\cite{Iyengar2023Sim2RealCTR, Fang2022Sim2Real}). 

Especially in deformable object manipulation (DOM), more and more research has covered Sim2Real. Liu et al \cite{Fei2021ICRASim2Real} and Liang et al \cite{liang2023real} utilized dense information (i.e., point cloud) to conduct Sim2Real calibration of deformable soft tissue. Distributional embedding \cite{Rika2022BaySim2Real} is proposed to
represent deformable object state, which can benefit the Sim2Real calibration of material properties from dense and noisy real observation.
A KF-ADMM framework\cite{Mehrnoosh2022MarkerSim2Real}and GNN-VAE\cite{Mehrnoosh2023GNNVAESim2Real}  is proposed to calibrate the tissue phantom deformation represented by one specific inner point movement with a set of complete markers. 


\Tian{below states our work is the first to use sparse and incomplete data frame for Sim2Real learning}
While previous studies have explored Sim2Real research for robots with a dataset containing frames with dense information \cite{Fei2021ICRASim2Real,liang2023real,Rika2022BaySim2Real} or fixed DoFs \cite{Mehrnoosh2022MarkerSim2Real,Fang2022Sim2Real, Gomes2023Sim2RealTactile, peng2018sim} for training, none of them have touched the concept of Sim2Real transfer for a sequence of soft deformable surface deformation with infinite DoFs by only sparse and incomplete ground-truth information.


% a requirement that proves challenging when transferring knowledge to soft deformable surfaces with attached markers that may become obscured during deformation (Fig.\ref{figTeaser}). Instead of discarding incomplete frames outright, we propose a resilient Sim2Real transfer pipeline to effectively leverage each incomplete frame, facilitating easier data collection and precise training.

\subsection{Simulation-based Forward Kinematics for Soft Robotics}

The forward kinematics (FK) of soft robots poses a greater complexity than that of rigid robots, given the challenging nature of obtaining an accurate solution due to the intricate morphology. Consequently, simulation plays a crucial role in effectively modeling the forward kinematics of soft robots \cite{Renda2023TROModeling}.

 Co-rotational FEM \cite{Felippa2000FEM} is a popular choice to account for geometry nonlinearity. Duriez initially incorporated this method into the FK modeling of soft robots, and further improvements were made through a constraint-based approach that considers both actuation and contact \cite{Duriez2013ICRA}. This development stands as a key component of the Simulation Open Framework Architecture (SOFA) \cite{SoFA2012Book}. Subsequently, James M. Bern et al. introduced a forward simulation model based on FEM, utilizing a compressible NeoHookean material model as the deformation energy density of the element \cite{Bern2017IROS}. 


 Another popular approach for modeling the Forward Kinematics (FK) of soft robots involves a geometric perspective. The Piecewise Constant Curvature (PCC) method, as described in \cite{Robert2010IJRR_PCC_Review}, assumes that the curvature remains constant within specific segments or intervals. This method is employed to predict the intricate shape of soft manipulators. Renda et al. introduced a geometric variable-strain approach for modeling soft manipulators, and this approach has been incorporated into a MATLAB library known as SoRoSim \cite{Renda2020VSA, mathew2021matlab}, contributing to advancements in research within the field. Fang et al. proposed a geometry-based framework for calculating the deformation of soft robots within the linear material elasticity range \cite{Guoxin2020TRO}, later refining it with considerations for interaction \cite{Guoxin2022IROS}. The simulator has been improved in this paper to be used to collect datasets for training the deformation of SoRo-Mannequin II in virtual environment.
 
Later, the differentiability of the forward simulation draws the attention of researchers. Du et al. proposed DiffPD\cite{du2021_diffpd} to model the soft robot deformation in a differentiable way. Hu et al proposed ChainQueen, a differentiable simulator based on MLS-MPM to model the soft robot\cite{hu2019chainqueen}.

 
\subsection{Neural Network Based Inverse Kinematics for Soft Robotics}
Inverse Kinematics (IK) is the process of finding optimal input parameters for a soft robotic system, and there is a growing trend in leveraging the capabilities of neural networks (NN) to construct IK solvers. The strength of neural networks lies in their ability to develop arbitrarily complex forward/inverse kinematic models, depending on the availability of abundant sample data and accounting for sensory noise \cite{Thomas2018SoRoCtrlReview}.

One notable attempt at employing NN for learning the IK network is presented by A. Melingui et al \cite{Melingui2014IJCNN}, who proposed a distal supervised learning approach by inverting the Forward Kinematics (FK) network. Another approach, proposed by Giorelli et al \cite{Michele2013IROS_NNDirectIK}, involves using Feed Forward Neural Networks (FNN) to directly output cable tensions for non-redundant robots.

For redundant robotic systems, the iterative solver with a learned differentiable FK model is commonly employed to determine actuation parameters for achieving smooth trajectories \cite{Fang2022Sim2Real}. In this context, a differentiable model is built by capturing the quasi-static physics of a soft robot, and it is used in gradient-based optimization to identify optimal open-loop actuation parameters \cite{bern2020soft}.


==> tex/secNNFastIK.tex <==
\section{Preliminary: Neural Network Based Fast Inverse Kinematics Solver}
\label{secNNFastIK}

\Tian{This section is ready.}

The neural network-based fast inverse kinematics solver (called \textit{\textbf{Fast IK Solver}})  on the virtual platform, as shown in Fig.~\ref{figDataPreparation} utilizes the gradient-based solver to compute optimal actuation parameters based on the efficient forward passing and back-propagation on the neural deformation model.



\subsection{Neural Deformation Model on Virtual Platform}
\label{secNeuralDefModel}
To acquire the dataset to train our neural deformation model, we have built up a geometry-based simulator based on \cite{Guoxin2020TRO,Guoxin2022IROS} to collect the data. The whole simulation process can be seen in Fig.\ref{figDataPreparation}. By importing chamber and membrane models,  our simulator automatically generates two types of boundary conditions. The first type involves fixture nodes, denoted by red points, which are immobilized and cannot be displaced in any direction. The second type comprises attaching nodes, represented by blue points, analogous to the chamber design, where overhanging chambers are affixed on top of the base chambers. The geometry-base simulator with the boundary conditions, can undergo deformation driven by actuation parameters. During intermediate iterations, our simulator performs adaptive collision checking (update spring elements) and employs a collision response algorithm to iteratively adjust the membrane model until it reaches a collision-free state. After multiple iterations, the system's final state is visualized, highlighting intricate details of multi-chamber interaction. This visualization depicts three chambers deforming collectively, with clear plots of their cross sections illustrating the deformed state of both the outer surface elements and inner tetrahedron elements. After acquiring the deformed membrane, we proceed to cut the mesh along the back. The resultant cut mesh exhibits two boundary curves with distinct directions, making it homeomorphic to a disc shape. Subsequently, parameterization becomes feasible, allowing for the extraction of free-form surface descriptors, such as B-Spline Control Points, for dimension reduction.

While our geometry-based simulator is more efficient than the Finite Element Method (FEM), it falls short of meeting the real-time computational demands for shape and gradient, not to mention the time-consuming procedures involved in computing free-form surface descriptors. To ensure the efficiency of the Fast IK solver, we have established a simulation forward kinematics network (neural deformation model on the virtual platform) to replace the laborious deformation simulation and post-processing procedures.

Initially, a thorough dataset is produced through domain randomization on the simulator, followed by post-processing steps. Subsequently, the simulation forward kinematics network, utilizing Multilayer Perceptron (MLP), is trained to capture the correlation between actuation parameters and delta control points (refer to details in Sec.~\ref{secLearningSimFKExperiments}).

The development of this neural deformation model on the virtual platform is designed to create a proficient surrogate for the simulator. This facilitates rapid and effective forward and backward queries (Further details are provided in Appendix.\ref{Appendix:GradCompShapeLoss} 
\& \ref{Appendix:GradCompNerualDef}) of FastIK Solver, thereby ensuring that the FastIK solver functions with optimal efficiency.




\subsection{Gradient-based Iterative IK Solver on Virtual Platform}
\label{secGradientBasedIK}

% it is a highly non-linear problem with its objective (called \textit{\textbf{shape approximation loss}}) involving two characteristics: 1) The dimensionality of shapes is nearly indefinite. 2) The loss is coupled with not only shapes but also poses ($\mathbf{R},\mathbf{t}$) as shown in Eq.\ref{eqLoss}. 

% \begin{equation}\label{eqLoss}
% \small
% D(\mathcal{T}(\mathbf{R},\mathbf{t}),\mathcal{S}(\mathbf{a})) = \sum_{j=1}^{n}  \left\| \hat{\mathbf{p}}_j - \left(\mathbf{R} \mathbf{c}^{\mathcal{T}^*}_j + \mathbf{t} \right) \right\|^2
% \end{equation}



% Where $\hat{\mathbf{p}}_j$ is the vertex on the deformed shape $\mathcal{S}$ and $\mathbf{c}^{\mathcal{T}^*}_j$ is the closet vertex of $\hat{\mathbf{p}}_j$ on the target shape $\mathcal{S}^T$.

% In our previous work \cite{Tian2022SoRoMannequin}, we proposed a model-free optimizer with the gradient (with respect to $\mathbf{a}$) calculated from hardware numerical differentiation \cite{Tian2022SoRoMannequin,Yip2014TROHardwardGradient}, which means the system jacobian is estimated through recording the surface shapes with locally changed actuation for each actuator, resulting in a time-consuming gradient evaluation process.

% What's worse, with the number of actuators increasing, the time used to calculate the gradient is increasing tremendously.

% To achieve more accurate and efficient 
% optimization, we propose a learning-based inverse kinematics framework with the gradient from differentiating the neural deformation model.

The \textit{\textbf{shape approximation loss}} of the FastIK solver can be defined as:

\begin{equation}\label{eqLoss}
\small
D(\mathcal{T}(\mathbf{R},\mathbf{t}),\mathcal{S}(\mathbf{a})) = \sum_{j=1}^{n}  \left\| \hat{\mathbf{p}}_j - \left(\mathbf{R} \mathbf{c}^{\mathcal{T}^*}_j + \mathbf{t} \right) \right\|^2
\end{equation}

Where $\hat{\mathbf{p}}_j$ is the vertex on the deformed shape $\mathcal{S}$ and $\mathbf{c}^{\mathcal{T}^*}_j$ is the closet vertex of $\hat{\mathbf{p}}_j$ on the target shape $\mathcal{S}^T$.

This is a highly nonlinear problem with no straightforward analytical solution considering: 1) The dimensionality of shapes is nearly indefinite; 2) The loss is coupled with not only actuation but also poses ($\mathbf{R},\mathbf{t}$). As a result, we propose an efficient gradient-based iterative IK solver (FastIK Solver) to address this issue, alternately updating actuation parameters and the transformation matrix (see Alg.~\ref{algInverseKinematic} and Fig.~\ref{figDataPreparation}).

For updating the actuation parameters, we efficiently evaluate the objective 
function and its gradient (to actuation) by forward passing and back-propagating the neural deformation model respectively. Then, the soft line search method is adopted to determine the next step~\cite{Guoxin2020TRO} of the actuation. The whole actuation updating will continue until no suitable step size can be determined, signaling the calculation of a new transformation. After several rounds of iteration, the optimal actuation, coupled with the transformation, can be achieved.

Our Fast IK solver could achieve much more efficient calculation (results in Sec.~\ref{secFastIKEfficiency}) compared with our previous IK solver~\cite{Tian2022SoRoMannequin} considering we could efficiently evaluate this analytical gradient instead of the finite difference one in the actuator space by hardware differentiation~\cite{Tian2022SoRoMannequin, Yip2014TROHardwardGradient}. 



==> tex/secResults.tex <==
%\section{Experimental Results}\label{secResults}

\subsection{Learning for Simulation Forward Kinematics}
\label{secLearningSimFKExperiments}
The primary objective of this first experiment is to determine the suitable representation for the output of Simulation Forward Kinematics (FK) Network.
As shown in Fig.\ref{figSimRepComp}(a), an MLP with two hidden layers with 128 neurons in each layer is selected to model the correlation between actuation parameters and surface shape. 

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figSimRepComp.jpg}\\
\vspace{-2pt}
\caption{Our simulation FK network is based on MLP to learn the mapping between actuation parameters and surface deformation, which can be described as three different kinds of representation: vertex-based, control-points-based, and delta-control-points-based. We have tested the performance of these representations in the test set （need to show the dataset） and the results are drawn in (a) \& (b). The representation of spline control points can achieve much better accuracy than the vertex-based representation. Furthermore, the delta control points, which are calculated by offsets from the undeformed control points, show even superior performance.}\label{figSimRepComp}
\end{figure}

The findings indicate that, rather than directly capturing the relationship between actuation parameters and vertex positions (which results in larger errors, as shown in Fig.\ref{figSimRepComp}(b)), an effective approach is to employ delta control points, which represent the displacement from the current control points to the locations of the undeformed control points. In short, the network is trained to learn these control point offsets. In our ablation study presented in Fig.\ref{figSimRepComp}, it is evident that the average point-to-mesh distance error is significantly reduced from 4.99 mm and 1.74 mm to 0.75 mm (an 84.97 \% reduction). Likewise, the average point-to-mesh maximum error decreases from 21.11 mm and 15.01 mm to 4.47 mm (a reduction of 78.83 \%). In summary, we consistently utilize delta control points as the simulation representation throughout the paper.


\subsection{Field Learning for Surface Sim2Real}
\label{secSim2RealResult}

% \Tian{This section needs to be rewritten to make it more compact}
The field learning approach for Surface Sim2Real can take two architectural routes. The first one, referred to as \textit{Naive Field Learning for Surface Sim2Real}, involves directly mapping from the simulation field to the real field using MLP, as illustrated in Fig.\ref{figFieldPipeline}(b). On the other hand, the second approach, known as \textit{RBF Field Learning for Surface Sim2Real}, entails initially learning the simulation field to function space through MLP. Subsequently, the relationship from the simulation field to the real field is established using differentiable space warping, as depicted in Fig.\ref{figFieldPipeline}(a). We will undertake a series of experiments to validate the following characteristics: 1) The capability of even a naive field learning network to calibrate simulation nonlinearity and fabrication inaccuracy. 2) The superiority of our RBF field learning architecture compared to the naive field learning architecture.

\subsubsection{Comparing Field Sim2Real Learning with a Simulation-only approach}


\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figReconLipExp.jpg}\\
\vspace{-2pt}
\caption{Calibrated Surface by Naive Field Sim2Real Network with Recon. Loss and Lip. Loss: (a), (b) \& (c): the Sim2Real network can successfully reduce simulation non-linearity and manufacturing imperfection.
}\label{figReconLip}
\end{figure}

The initial experiment aims to confirm the efficacy of the field learning architecture (even if it is the naive one as shown in Fig.\ref{figFieldPipeline}(b)) in rectifying the inaccuracy stemming from both simulation and fabrication. 

In our training process, we opt for the Reconstruction loss (Recon. Loss) and Lipschitz loss~\cite{liu2022lipLoss} (Lip. Loss) as the chosen loss functions. The former serves to guarantee Sim2Real accuracy introduced by captured markers, while the latter ensures the smoothness of the learned manifold.

In Fig.~\ref{figReconLip}, we have applied the same actuation parameters on the real physical prototype (SoRo-Mannequin II), the simulator, and the naive field Sim2Real Network to get the scanned model, simulation model, and calibrated model respectively. Further, the difference between the latter two models (simulation one and calibrated one) and the first model (scanned one as ground-truth information) have been measured and visualized.

As depicted in Fig.~\ref{figReconLip}(a), when all actuation parameters are set to zero, substantial errors are observed in the simulation model, particularly in the belly region. This discrepancy is attributed to the manufacturing imperfections arising from the additional layer thickness inherent in the three-layer design. 
Fortunately, our Field Sim2Real network adeptly captures this phenomenon, as evidenced by a notable reduction of $18.5\%$, $20.2\%$, and $23.1\%$ in maximum error, average error, and standard deviation, respectively. When applying a distinct actuation vector (reaching maximum threshold) as shown in Fig.~\ref{figReconLip}(b), our naive field Sim2Real network exhibits significantly improved accuracy, achieving reductions of $27.1\%$, $51.4\%$, and $36.5\%$ in maximum error, average error, and standard deviation compared to the simulation result. In the final case, illustrated in Fig.\ref{figReconLip}(c), the average error experiences a large reduction of $32.9\%$. It is truly promising to note that the field Sim2Real network effectively narrows the reality gap.

\subsubsection{Comparing RBF Field Sim2Real Network with the Naive Field Sim2Real Network}
\label{secRBFFieldLearningResult}
%this table is too long, move to separate tex file
\input{tex/TableI}


To verify the effectiveness of our RBF Field Sim2Real network as shown in Fig.\ref{figFieldPipeline}(a) compared to the naive field learning network (Fig.\ref{figFieldPipeline}(b)), we have conducted a series of experiments.

The naive field learning network encompasses various types based on loss functions and activation functions. The initial baseline employs reconstruction loss (Recon. Loss) as the loss function and ReLU as the activation function. The second baseline involves incorporating an additional Lipschitz regularization (Lip. Loss) term~\cite{liu2022lipLoss} into the total loss during the training process. The third and ultimate baselines use reconstruction loss exclusively, but substitute ReLU with the Siren activation function~\cite{sitzmann2020implicit} and RBF activation function~\cite{nabney2004efficientRBFNN}, respectively. Our proposed RBF Field Network was compared with these four baselines. 

Firstly, the $C^1$ continuity and smoothness properties of the learned field from these different field learning networks were examined. $C^1$ continuity measures whether the shape gradient is continuous on the surface, while smoothness $S_i$ on the mesh vertex $i$ is defined as the norm of the gradient of the Laplacian~\cite{Sorkine2005Laplacian} norm to approximate the magnitude of surface geometry changes:

% \begin{equation}\label{eqSmoothness}
% \small
% D(\mathcal{T}(\mathbf{R},\mathbf{t}),\mathcal{S}(\mathbf{a})) = \sum_{j=1}^{n}  \left\| \hat{\mathbf{p}}_j - \left(\mathbf{R} \mathbf{c}^{\mathcal{T}^*}_j + \mathbf{t} \right) \right\|^2
% \end{equation}

\begin{equation}\label{eqSmoothness}
 S_i = \norm{\nabla \norm{\delta_{i}}}
 = \| \nabla \| \frac{1}{d_i} \sum_{j\in N(i)} (\overrightarrow{V_{i}}-\overrightarrow{V_{j}}) \| \|
\end{equation}

The higher value of $S_i$ indicates a rougher surface, possibly featuring wrinkles.

In Fig.\ref{figFieldProperty}(a), we have applied the same actuation parameters on five field learning methods and acquired the output calibrated models. The Naive Field Learning approach, employing only Reconstruction Loss (A), fails to produce a continuous gradient in the output field, evident from the surface wrinkles. For the smoothness evaluation, the surface wrinkles (A) have been faithfully highlighted by the red region in Fig.\ref{figFieldProperty}(a) where the local shape is changing dramatically. It is obvious that the Naive Field Learning approach with additional Lip. Loss (B) is still producing a large unsmooth shape. However, the naive field network with Siren activation function, the naive field with RBF activation function, and our proposed RBF field network are capable of creating fields with similar smoothness. 

 
 Moreover, We applied four distinct actuation parameters to the physical setup and compared the scanned mesh with the output of these five methods to calculate both mean and maximum errors. The summarized results can be found in Tab.~\ref{tab:fieldLearningComparison}, and the error colormaps are detailed in Fig.\ref{figFieldProperty}(b-d) where the maximum value for the color bar is 15mm. The statistics and the colormap show our RBF field network for surface Sim2Real has achieved exceptional performance in all cases, largely reducing mean error and maximum error. 
 
 Furthermore, the properties of these field learning architectures are summarized in Table.~\ref{tab:fieldLearningComparison}. Note that considering the naive field learning network with Recon. Loss can not output the $C^1$ Continuity field, we didn't calculate the mean and maximum error of the output meshes of this network to the scanned models. In conclusion, the proposed RBF field learning network is the only field learning network to simultaneously satisfy all three requirements: $C^1$ continuity, local shape smoothness and small reality gap.
 


\subsubsection{The Capability of RBF Field Network to Satisfy All Fundamental Requirements}
The proposed RBF Field Network can satisfy all the fundamental requirements listed in Sec.~\ref{secRequirement}. 


For \textit{\textbf{the first requirement}} which asks for the learning framework can deal with a modest dataset from hardware with incomplete frames, the training set for our RBF field learning framework only includes 43 frames as shown in Fig.\ref{figDataset}. What's more, we have plotted the available markers and total markers for each frame to further illustrate the details of information loss. 

\textit{\textbf{The second requirement}} 
asks for the sparsity of the training data. Compared to the dimension of the surface descriptor with 900 control points (equivalent to 2700 DoFs), the dimension of the captured markers DoFs is much lower (around 90 DoFs). We have further plotted the percentage of markers' DoFs relative to surface descriptors' DoFs in Fig.~\ref{figDataset}, which is around 3 $\%$. \textit{\textbf{The second requirement}} also asks for the learned framework can be generalized to unseen case. In Fig.~\ref{figFieldProperty}, for case I to case III, these shapes are related to actuation parameters that are not included in the training dataset, but the MLP has successfully learned RBF function space, which further corrected the Sim2Real transfer with error to scanned model largely reduced.

For \textit{\textbf{the third requirement}} that asks for the Sim2Real pipeline to be in an end-to-end manner, our RBF field network is fully differentiable with its end-to-end gradient derived in Appendix.\ref{Appendix:GradCompShapeLoss} 
\& \ref{Appendix:GradCompNerualDef}. To show the computational cost of the shape approximation loss ($D$) calculation and its gradient ($\frac{\partial D}{\partial \textbf{a}}$) evaluation during the forward pass and backward pass by the chain rule as shown in Fig.~\ref{figVarRelation}, a comprehensive table has been illustrated the detailed time consumption. From the Table.~\ref{tab:rbfFieldCompTime}, the forward pass takes 27.8 ms while the backward pass takes 54.6 ms. It is interesting to note that if we use the finite difference on the network to approximate the analytical gradient, it will take $(9 + 1) * 27.8 = 278.0$ ms, which is nearly 3.4 times that of our analytical one. This table shows the ability of our RBF Field Network to efficiently conduct forward pass and back-propagation to acquire the free-form surface shape and its gradient in an end-to-end manner, facilitating the efficient Sim2Real computation and FastIK solver.

\input{tex/TableTimes}

For \textit{\textbf{the fourth requirement}} that asks for smooth and accurate Sim2Real transfer, we have validated these characteristics in Sec.~\ref{secRBFFieldLearningResult} and Table.~\ref{tab:fieldLearningComparison}.


% \subsubsection{Tradition Sim2Real Learning with Space Warping}
% \Tian{Add traditional field learning: discard missing markers across the whole captured sequence and learn the actuation-marker relationship. In each test, linear solve each frame to get the calibrated result and compare with the scanned result. }
% \Tian{This experiment is important to demonstrate the advantage of our solve to make use of the whole dataset. To do in Jan-06-2024}
%\Tian{This one maybe not necessary}


% \subsubsection{Naive Field Learning for Surface Sim2Real}
% \label{secNaiveField}



% The naive field learning pipeline (in Fig.\ref{figFieldPipeline}(a)) directly predicts the calibrated point $\mathbf{\hat{q}}_{sj}$ by feeding the query point $\mathbf{q}_{sj}$ and encoded $\mathbf{Z}$ vector into the network. In this section, four baselines using different activation functions and loss functions are implemented to test the Sim2Real error. 

% The first baseline is finished by only imposing reconstruction loss, and the trained field can be visualized by feeding simulation vertices into the trained network and constructing the calibrated mesh as shown in Fig.~\ref{figReconOnly}, which shows the field is non-smooth across the whole domain.

% \begin{figure}[h] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figReconLossOnly.jpg}\\
% \vspace{-2pt}
% \caption{Calibrated Surface by Naive Field Sim2Real Network with Recon. Loss only.
% }\label{figReconOnly}
% \end{figure}



% The second baseline is adding one extra Lipschitz regularization term \cite{liu2022lipLoss} into total loss in the training process. In the
% Fig.~\ref{figReconLip}, we have applied different actuation parameters on the real physical prototype, simulation platform, and naive field Sim2Real Network with Recon. and Lip. Loss. In Fig.~\ref{figReconLip}(a) where all actuation is set to zero, the simulation result has large errors around the belly region considering our three-layer design brought manufacturing imperfection (increase the membrane thickness). It is exciting to observe that the naive field network for surface Sim2Real can still adjust the simulation and manufacturing inaccuracy (indicated by the maximum error, average error, and standard deviation reduced by $18.5\%$, $20.2\%$, and $23.1\%$ respectively). In Fig.~\ref{figReconLip}(b), with maximum actuation applied on setup, it is further observed that our naive field Sim2Real network (with Recon. and Lip. Loss.) can achieve much better accuracy with $27.1\%$, $51.4\%$, and $36.5\%$ reduction on the maximum error, average error, and standard deviation compared to the simulation result.

% However, this naive field NN (with Recon. Loss and Lip. Loss) can not faithfully preserve local shape smoothness as shown in Fig.~\ref{figLipSmoothVar}(a), especially in the zoom-in areas. What's more, the laplacian (\cite{Sorkine2005Laplacian}) gradient norm is drawn in colormap and histogram to validate this conclusion.


% \begin{figure}[h] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figLipSmoothVariation.jpg}\\
% \vspace{-2pt}
% \caption{Calibrated Surface by Naive Field Sim2Real Network with Recon. Loss and Lip. Loss: (a) it cannot preserve local shape property, the local shape detail variation is changing dramatically as shown in (b) where a larger value indicates the worsened shape preserving. 
% }\label{figLipSmoothVar}
% \end{figure}



% The third baseline is the naive field NN with Recon. Loss and Siren activation function \cite{sitzmann2020implicit}. In Fig.~\ref{figReconSiren}(d), the siren activation function could achieve better smoothness-preserving than NN with Lip. Loss. However, its Sim2Real error is still undesirable when the deformable mannequin has a large inflation shape: around $14.8\%$  (Fig.\ref{figReconSiren}(b)) and $17.6\%$ (Fig.\ref{figReconSiren}(c)) increase on the average error compared to results with NN of Lip. Loss.

% \begin{figure}[h] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figReconSirenExp.jpg}\\
% \vspace{-2pt}
% \caption{Calibrated Surface by Naive Field Sim2Real Network with Recon. Loss and Siren Activation: (d): Siren activation can improve the local shape preserving but can not improve Sim2Real error to the level of NN with Lip. Loss (a-c).
% }\label{figReconSiren}
% \end{figure}


% The final baseline is the naive field Sim2Real NN with RBF activation function~\cite{nabney2004efficientRBFNN} with its parameters tuned during the training. After training, we visualize its sim2real error in Fig.~\ref{figReconRBFNaive}(a-c), the sim2real error is increased tremendously, especially the average error for Fig.~\ref{figReconRBFNaive}(b) and (c) with 7.09 mm ($63.8\%$) and 3.98 mm ($27.0\%$). The property comparison is listed in Table. ~\ref{tab:naiveFieldComparison}.

% \begin{figure}[h] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figReconRBFLayerExp.jpg}\\
% \vspace{-2pt}
% \caption{Calibrated Surface by Naive Field Sim2Real Network with Recon. Loss and RBF Layer: (d): RBF layer can improve the local shape preserving but can not improve Sim2Real error to the level of NN with Lip. Loss (a-c).
% }\label{figReconRBFNaive}
% \end{figure}









% \subsubsection{RBF Field Learning for Surface Sim2Real}
% The naive field learning networks (as shown in Fig.~\ref{figFieldPipeline}(a)), which directly learn the field-to-field relationship with different activation and loss functions, however, are not capable of simultaneously satisfying the requirements of $C^{1}$ continuity, a local smoothness-preserving property, and a small Sim2Real error. 

% \begin{figure}[h] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figRBFSim2Real.jpg}\\
% \vspace{-2pt}
% \caption{Calibrated Surface by RBF Field Sim2Real Network: (d): this network can better achieve the local shape preserving and also be able to reduce Sim2Real error compared to the best performed naive Field Sim2Real with Recon. Loss and Lip. Loss.
% }\label{figReconRBFSim2Real}
% \end{figure}

% On the contrary, our RBF Field Learning Network for Surface Sim2Real as shown in Fig.\ref{figFieldPipeline}(b), can achieve more accurate and robust calibrated results across all shapes. Especially when it is with fat shapes, our proposed pipeline reduces the maximum error by $23.2\%$, $33.7\%$ and $50.4\%$ respectively in Fig.~\ref{figReconRBFSim2Real} (a-c). Furthermore, it can achieve local smoothness preserving as shown in Fig.~\ref{figReconRBFSim2Real} (d) with an average value reduced by $36.4\%$ and a maximum value reduced by $45.0\%$.

% \begin{table}[h] \footnotesize%\tiny %scriptsize
% %\footnotesize
% \centering


% \begin{tabular}{cc|c|c|c}         %adjust column number 
% \hline \hline                       %horizontal line
% \specialrule{0em}{2pt}{1pt}         %vertical space
% \multicolumn{2}{c|}{\multirow{2}{*}{\textit{}~}}  & \multicolumn{3}{c}{Property} \\ %column arrangement
% \specialrule{0em}{1pt}{2pt}         %vertical space
% \cline{3-5}                        %segementation line
% \specialrule{0em}{2pt}{1pt}         %vertical space

% % \multicolumn{2}{c|}{\multirow{2}{*}{\textit{}~}}  
% \multicolumn{2}{c|}{Network Type}  
% % & \multicolumn{1}{c|}{Shape $C^1$ Continuity} & \multicolumn{1}{c|}{Local Shape Preserving}  & \multicolumn{1}{c}{Small Sim2Real Error} 
% & \multicolumn{1}{c|}{Type A$^\dagger$} & \multicolumn{1}{c|}{Type B$^\star$}  & \multicolumn{1}{c}{Type C$^\ddagger$} 
% \\ 

% %Recon. Only: \ding{55} is wrong, \ding{51} is right
% \specialrule{0em}{1pt}{2pt}
% \hline \specialrule{0em}{1pt}{2pt}
% \multicolumn{2}{c|}{Naive Field (Recon.)} & \color{red}\ding{55} & \color{red}\ding{55} & \color{red}\ding{55}\\

% \specialrule{0em}{1pt}{2pt}
% \hline \specialrule{0em}{1pt}{2pt}
% \multicolumn{2}{c|}{Naive Field (Recon. + Lip.)} & \color{blue}\ding{51} & \color{red}\ding{55} & \color{blue}\ding{51}\\

% \specialrule{0em}{1pt}{2pt}
% \hline \specialrule{0em}{1pt}{2pt}
% \multicolumn{2}{c|}{Naive Field (Recon. + Siren)} & \color{blue}\ding{51} & \color{blue}\ding{51} & \color{red}\ding{55}\\

% \specialrule{0em}{1pt}{2pt}
% \hline \specialrule{0em}{1pt}{2pt}
% \multicolumn{2}{c|}{Naive Field (Recon. + RBF Layer)
% } & \color{blue}\ding{51} & \color{blue}\ding{51} & \color{red}\ding{55}\\

% \specialrule{0em}{1pt}{2pt}
% \hline \specialrule{0em}{1pt}{2pt}
% \multicolumn{2}{c|}{\color{blue} RBF Field Sim2Real (Ours)
% } & \color{blue}\ding{51} & \color{blue}\ding{51} & \color{blue}\ding{51}\\

% \specialrule{0em}{0pt}{2pt} \hline\hline
% \end{tabular}

% \begin{flushleft}\scriptsize
% $^\dagger$ $C^1$ Continuity: measure whether the shape gradient is continuous on the surface.\\
% $^\star$ Local Shape Smoothness: measure whether the local shape is changing dramatically.\\
% $^\ddagger$ Small Sim2Real Error: measure the Sim2Real transfer ability to reduce error.\\
% \end{flushleft}

% \caption{Comparison of Different Field Learning Network Performance.\Tian{This table should be shown close to other figures to compress the space occupied}}\label{tab:naiveFieldComparison}
% \vspace{-10pt}
% \end{table}

% \subsubsection{Tradition Sim2Real Learning with Space Warping}
% \Tian{Add traditional field learning: discard missing markers across the whole captured sequence and learn the actuation-marker relationship. In each test, linear solve each frame to get the calibrated result and compare with the scanned result. }
% \Tian{This experiment is important to demonstrate the advantage of our solve to make use of the whole dataset. To do in Jan-06-2024}

\subsection{Inverse Kinematics Results}
\label{secIKResults}



\subsubsection{Shape Approximation Results}
We have applied the neural network-based IK solver to four different target models selected from CAESAR dataset \cite{} and set the converged condition as: 

\begin{equation}\label{eqTerminalCond}
%\frac
\frac{|D(\mathcal{T},\mathcal{S}(\mathbf{a}_{i+1}))-D(\mathcal{T},\mathcal{S}(\mathbf{a}_i))|}{D(\mathcal{T},\mathcal{S}(\mathbf{a}_{i+1}))} \leq \tau
\end{equation} 
with $\tau=1\%$ are used in this paper.

The progressive results have been visualized in Fig.\ref{figIKResult}. The error curve has been plotted to show the whole iteration process. To have a better illustration for the free-form surface shape approximation during iteration, we have drawn two wireframes (red to represent the deformed shape by our Neural Deformation Model and blue to demonstrate the target model with its transformation matrix adjustable) for Iter $\#1$, Iter $\#5$ and Iter $\#30$. These figures vividly demonstrate the success of our Neural network-based IK solver in approximating the provided target shapes, incorporating relative poses in the iterative process.

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figProgressiveResult.jpg}\\
\vspace{-2pt}
\caption{The Progressive results by the proposed Fast IK Solver: The whole process is plotted with three intermediate iterations to validate our algorithm. We further scanned the deformed surface and compared it to the target model with error colormap to verify the correctness of our Sim2Real learning and FastIK solver.
}\label{figIKResult}
\end{figure}

We further scanned three intermediate shapes during iterations to demonstrate our Sim2Real framework has achieved promising results to bridge the reality gap. A final converged shape has been scanned and visualized by error colormap by finding its closest distances to the target mesh. The colormap has an average error and maximum error at about 6.16 mm and 22.97 mm respectively, which shows the promising fitting ability of our SoRo-Mannequin II.

In order to highlight the importance of Sim2Real transfer in bridging the reality gap, we conducted one experiment (FastIK without Sim2Real) to acquire the optimal actuation and apply it to the physical setup. The obtained actuation (from FastIK without Sim2Real) showed the worse fit compared to the one with Sim2Real, which can be seen in Fig.\ref{figIKwithoutSim2RealResult}.

\begin{figure}[t] 
\centering
\includegraphics[width=0.95\linewidth]{fig/figFastIKwithoutSim2Real.jpg}\\
\vspace{-2pt}
\caption{We conducted an ablation study to confirm the significance of our Sim2Real method in enhancing the FastIK results. The simulation struggles to well capture real deformation caused by manufacturing imperfections and simulation nonlinearity. However, our Sim2Real method effectively addresses this challenge, further facilitating precise shape approximation to the target model $M3$.
}\label{figIKwithoutSim2RealResult}
\end{figure}


Furthermore, it's exciting to note that the proposed Fast IK solver has yielded positive outcomes across all four target models.

As shown in Fig.\ref{figAllResults}, our FastIK solver can achieve a nice approximation to different target models with a large variation in body dimensions. The average error and maximum error for each approximation task can be found in Table.\ref{tab:IKstatistics} (unit is mm).





\begin{figure*}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figAllResults.jpg}\\

\vspace{-2pt}
%%%%%%%%%%%%%%%%%%%
% \scriptsize %\tiny \scriptsize \footnotesize \small
% \begin{tabular}{c|c|c|c|c}
% \hline
% \textbf{Models:} & $M1$ & $M2$ & $M3$ & $M4$ \\ 
% \hline\hline
% \textbf{Average Err.: $\frac{1}{n}\sum_{j=1}^n \| \mathbf{p}_j - \mathbf{c}^{\mathcal{T}}_j \|$} & $3.85$ & $5.72$ & $6.16$ & $5.25$ \\ 
% \hline 
% \textbf{Max. Err.: $\max_{j=1, \ldots, n} \| \mathbf{p}_j - \mathbf{c}^{\mathcal{T}}_j \|$} & $16.37$ & $23.24$ & $22.97$ & $17.68$ \\ 
% \hline 
% \end{tabular}

\vspace{-2pt}
\caption{The final results of approximating four different target models by a side-by-side comparison.
}\label{figAllResults}
\end{figure*}


\begin{table}[t]\footnotesize
\centering
\caption{The error colormap of the final results. (unit: mm)}
\scriptsize %\tiny \scriptsize \footnotesize \small
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Models:} & $M1$ & $M2$ & $M3$ & $M4$ \\ 
\hline\hline
\textbf{Average Err.: $\frac{1}{n}\sum_{j=1}^n \| \mathbf{p}_j - \mathbf{c}^{\mathcal{T}}_j \|$} & $3.85$ & $5.72$ & $6.16$ & $5.25$ \\ 
\hline 
\textbf{Max. Err.: $\max_{j=1, \ldots, n} \| \mathbf{p}_j - \mathbf{c}^{\mathcal{T}}_j \|$} & $16.37$ & $23.24$ & $22.97$ & $17.68$ \\ 
\hline 
\end{tabular}
\label{tab:IKstatistics}
\end{table}


\subsubsection{Efficiency Comparison}
\label{secFastIKEfficiency}

To assess the efficiency of the proposed FastIK solver in comparison to our previous model-free method \cite{Tian2022SoRoMannequin}, we conducted several experiments to compare the time consumption using these two methods and collect the data in Table.~\ref{tab:CompStatistics}.


\begin{table}[t]\footnotesize
\centering
\caption{Time Costs on Physical Platform}
\begin{tabular}{c|c|c|c|c}
\hline\hline
\textbf{Models} & $M1$ & $M2$ & $M3$ & $M4$ \\ 
\hline 
\hline 
\multicolumn{5}{c}{Hybrid Solver (Baseline Method $^\dag$)}\\
\hline 
\# of Steps & $14$ & $16$ & $16$ & $20$ \\ 
\hline 
Total Time (sec.) & $945.6$ & $1125.3$ & $1044.6$ & $1242.1$ \\ 
\hline 
\hline 
\multicolumn{5}{c}{Fast IK Solver with Robust Sim2Real Network (Proposed Method)}\\
\hline 
\# of Steps & $14$ & $8$ & $9$ & $8$ \\ 
\hline 
Total Time (sec.) & $7.9$ & $4.7$ & $5.6$ & $4.8$ \\ 
\hline 
\textcolor{blue}{Order of Improvement (times)} & \textcolor{blue}{$119.7$} & \textcolor{blue}{$239.4$}& \textcolor{blue}{$186.5$}& \textcolor{blue}{$258.8$}\\ 
\hline\hline
\end{tabular}
\begin{flushleft}
$^\dag$ The baseline is the model-free algorithm proposed in our previous paper \cite{Tian2022SoRoMannequin}. Note that $\tau=1.0\%$ and $i_{\max}=30$ are used in this experiment. 
\end{flushleft}\label{tab:CompStatistics}
\end{table}


From Table. \ref{tab:CompStatistics}, our solver can achieve much more efficient computation in all four target models with efficiency improved larger than two magnitudes. For Model M1, our solver only took 7.9 seconds to reach the converged state, which is 119.7 times faster compared to the baseline method with 945.6 seconds. For M2 and M3, our solver achieved 239.4 and 186.5 times faster than the baseline method respectively. For M4, our method could even achieve 258.8 times faster results. It's worth mentioning that our FastIK solver achieved efficient and robust approximation results in less than 8 seconds, which enables practical shape matching, benefiting diverse application scenarios. 

\input{tex/Alg}





==> tex/secSim2Real.tex <==
\section{Robust Sim2Real Transfer Learning}
\label{secSim2Real}

\Tian{This section is ready.}
The Fast IK solver, implemented on the virtual platform, relies exclusively on a neural deformation model with only simulation data, leading to inherent discrepancies with real-world scenarios as shown in Fig.~\ref{figTeaser}. Additionally, the ground-truth data obtained from vision devices exhibit instability, as depicted in Fig.~\ref{figTeaser}, with challenges such as 1) sparse and unstable marker capturing resulting in missing data, and 2) non-constant scanned geometry around the boundary. Consequently, we propose a robust Sim2Real transfer learning framework to enhance the FastIK solver. This framework aims to bridge the reality gap by leveraging \textit{\textbf{sparse}} and \textit{\textbf{incomplete}} ground-truth information (i.e., motion capture markers), facilitating the accurate capture of \textit{\textbf{sequential}} free-form surface morphing with dense Degrees of Freedom (DoFs).

% This underscores the considerable advantage of Sim2Real transfer learning.

% In this section, we will introduce our robust Radial-basis-function (RBF) Field Learning Network for Surface Sim2Real Transfer, using only limited and even incomplete ground-truth information to faithfully capture the soft free-form surface morphing that comes with nearly indefinite Degree-of-Freedoms (DoFs) to account for the simulation and fabrication inaccuracy. 



%reducing the need for extensive real-world data collection.

\subsection{Robustness Requirement}
\label{secRequirement}

Naturally, the common ideal is to learn the whole simulation surface shape to the whole real surface shape (fixed DoFs) mapping by MLP. However, there are several limitations exist in this architecture:

\begin{itemize}
    \item Requiring dense ground-truth information, along with the accurate correspondence among captured sequences.
    \item The data collection process is intricate, requiring assurance that each frame is complete without any partial information loss, the captured range matches the simulation, and there is a clear boundary.
    \item The involvement of tedious post-processing steps, including data cleaning and parameterization, adds to the complexity.
\end{itemize}

%Especially if we use the scanner to capture the ground-truth info, it is impractical to acquire the whole scanned mesh with perfect topology (e.g., has clear sharp features, no small holes, and no intersection), which is important to be processed to be B-Spline control points. For RGB-D devices that come with point clouds, it is hard to ensure the captured range is the same as the simulation one. Furthermore, the parameterization of point clouds is hard to consistent throughout the whole capture sequence (with different shapes). If we choose a dense marker set to provide a label, it will easily bring the problem of marker missing, which can not be solved by this architecture.

Rather than imposing stringent demands on data collection (Sim2Real values a straightforward and resilient data collection and training process), we relax some conditions and outline fundamental requirements for surface Sim2Real transfer:


\begin{itemize}
    \item Allow for frame incompleteness, accommodating partial information loss, and require only a modest dataset from the hardware.
    \item Embrace datasets with sparse information to facilitate the calibration of dense surface morphing with indefinite Degrees of Freedom (DoFs). The Sim2Real transfer once learned, can be generalized to unseen cases.
    \item The transfer should be in an end-to-end manner.
    \item The surface after Sim2Real transfer should be smooth and accurate compared to the ground-truth one.
\end{itemize}



\subsection{Elastic Space Warping for Surface Sim2Real}\label{secElasticWarping}

Elastic Space Warping \cite{Charlie2007RBFVolPara} proves to be a potent tool for creating a nonlinear mapping between two fields (a simulation field comprises the simulation model and a real field contains the real model). This is achieved by providing two corresponding sets of sparse anchor points in simulation and reality respectively, making it well-suited for integration into our Sim2Real transfer approach. The illustration is drawn in Fig.\ref{figSpaceWraping}.



The equation for the elastic space warping can be listed:

\begin{equation}
\label{equRBF}
    \mathbf{\hat{q}}_{sj} = \mathbf{\Phi}(\mathbf{q}_{sj}) = \mathbf{a_{0}} + \mathbf{A}\mathbf{q}_{sj} +
   \sum_{i=1}^{N} \mathbf{b}_i g(\mathopen| \mathbf{q}_{sj} - \mathbf{q}_{i} \mathclose|)
\end{equation}


where
\begin{equation}
\label{equA}
\mathbf{A}=
\bigg[\begin{array}{c|c|c}
\mathbf{a}_1 &\mathbf{a}_2 &\mathbf{a}_3
\end{array}\bigg]
\end{equation}

In this equation, $\mathbf{q}_{sj}$ denotes a point on the simulation surface within the \textit{\textbf{simulation field}}, while $\mathbf{\hat{q}}_{sj}$ represents the point on the calibrated model within the \textit{\textbf{real field}} acquired through Sim2Real. In our case, $\mathbf{q}_{i}$ is the simulation marker (also called anchor point) corresponding to the real motion capture marker.


The mapping $\mathbf{\Phi}$ between these two fields is parameterized by a set of basic vectors ($\mathbf{a}_0$, $\mathbf{a}_1$, $\mathbf{a}_2$, $\mathbf{a}_3$ and $\mathbf{b}_i$ as column vector). $\bm{\gamma}$ (named function space variables) is used to encapsulate them.

Some weightings of the function space variables are radial basis function $g(\mathopen| \mathbf{q}_{sj} - \mathbf{q}_{i} \mathclose|)$ (where $g(*)$  is chosen to be Gaussian $\phi(r) = e^{-cr^2}$  \cite{Carr2001RBF}). 
%$\{\mathbf{q}_{i}\}$ represents the simulation marker sets. 
Eq.\ref{equRBF} stands for transforming any simulation point $\mathbf{q}_{sj}$ in the simulation field with the summation of all gaussian kernels' values at $\mathbf{q}_{sj}$ (i.e., $\sum_{i=1}^{N} \mathbf{b}_i g(\mathopen| \mathbf{q}_{sj} - \mathbf{q}_{i} \mathclose|)$), plus a linear offset (i.e., $\mathbf{a_{0}} + \mathbf{A}\mathbf{q}_{sj}$), to yield the corresponding points $\mathbf{\hat{q}}_{sj}$ in the real field. The illustration of the summation can be found on the right-hand side of Fig.~\ref{figSpaceWraping}.

As for how to solve the function space variables, by utilizing two sets of sparse anchor points  ($\{\mathbf{q}_{i}\}$ represents the simulation marker sets and $\{\hat{\mathbf{q}}_{i}\}$ represents the captured real marker locations), the field mapping $\mathbf{\Phi}$ can be computed by solving a linear system as outlined below:


\begingroup
\begin{equation}\label{eqWarpingFunc}
\begin{aligned}
\left[
 \begin{matrix}
   g_{11} & g_{12}  &...&g_{1N}&1&\mathbf{q}_{1}^T\\
   g_{21} & g_{22}  &...&g_{2N}&1&\mathbf{q}_{2}^T\\
   \vdots & \vdots  &\ddots & \vdots & \vdots & \vdots \\
   g_{N2} & g_{N3}  &...&g_{NN}&1&\mathbf{q}_{N}^T\\
   1      & 1       &...&1     &\mathbf{0}&\mathbf{0}\\
   \mathbf{q}_{1} & \mathbf{q}_{2}&...&\mathbf{q}_{N}&\mathbf{0} &\mathbf{0}
  \end{matrix}
  \right] 
  \left[
   \begin{matrix}
   {\mathbf{b}_1}^{T} \\ {\mathbf{b}_2}^{T} \\ \vdots  \\{\mathbf{b}_{N}}^{T} \\ {\mathbf{a}_0}^{T}\\ {\mathbf{a}_1}^{T}\\ {\mathbf{a}_2}^{T}\\ {\mathbf{a}_3}^{T}
   \end{matrix}
   \right]
   = 
   \left[
   \begin{matrix}
    {\mathbf{\hat{q}}_{1}}^T \\ {\mathbf{\hat{q}}_{2}}^T \\ \vdots  \\{\mathbf{\hat{q}}_{N}}^T \\ \mathbf{0}\\ \mathbf{0}\\\mathbf{0}\\ \mathbf{0}
   \end{matrix}
   \right]
\end{aligned}
\end{equation}
\endgroup

Where $ g_{ij} = g(\mathopen| \mathbf{q}_{i} - \mathbf{q}_{j} \mathclose|)$ denotes the radial basis function for given markers $\mathbf{q}_{i}$ and $\mathbf{q}_{j}$ in the simulation field.

The solved function space variable $\bm{\gamma}$, however, is only feasible for the single simulation surface shape and can not be applied to a sequence of surface shapes (as shown in the left-hand side of Fig.~\ref{figSpaceWraping}), which is particularly important in our neural deformation model since it is expected to learn the whole shape space instead of the single shape point. As a result, we further propose to leverage the power of the network to learn the relationship between simulation shape spaces and function space, facilitating continuous function space variables corresponding to varying simulation shapes.

\subsection{RBF Field Learning for Surface Sim2Real}

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figFieldLearning.jpg}\\
\vspace{-2pt}
\caption{ 
(a) Our proposed RBF Field Learning Framework firstly learns the relationship between surface descriptor (simulation delta control points) and function space variables by MLP. Then, a field Sim2Real calibrates every single point in the simulation field to the real field by differentiable space warping. This approach outperforms (b) the naive Field Sim2Real Network, which relies solely on an MLP to directly learn the implicit field.\Tian{Update symbol explanation}
}\label{figFieldPipeline}
\end{figure}

% Two different types of field Sim2Real Transfer Network: (a) Naive Field Sim2Real Transfer. The input of the Sim2Real Network contains two parts: 1) simulation position on the simulation surface and 2) encoded latent code Z which further compresses the information of surface to low-dimension space. For each input simulated surface point, our NN will output the calibrated point on the real surface. 

The elastic space warping provides an opportunity to take advantage of sparse information to conduct Sim2Real transfer. However, It still can not fulfill the basic requirements detailed in Sec.\ref{secRequirement} considering there still exist three limitations:
\begin{itemize}
    \item The linear system necessitates the complete set of markers, posing a challenge to \textit{\textbf{the first requirement}}.
    \item The linear system must be solved each time for a new deformed surface shape to obtain coefficients, leading to time consumption and posing a challenge to \textit{\textbf{the second requirement}}.
    \item It cannot be directly integrated into our neural deformation model as it lacks an end-to-end solution, presenting a conflict with \textit{\textbf{the third requirement}}.
\end{itemize}

These limitations are very critical since they highly increase the workload for dataset collection. Actually, it cannot be inserted into the IK framework: a) The framework needs to be back-propagated to get an end-to-end gradient as a whole; b) The solved RBF coefficients are only feasible to the single case, which can not be generalized to a sequence of simulation fields including unseen cases. 

 Combining with these limitations and robust requirements listed in Sec.\ref{secRequirement}, we reformulate the sim2Real transfer problem as the \textit{\textbf{implicit field learning}} problem and propose a novel implicit learning framework (\textit{\textbf{RBF Field Learning Network for Surface Sim2Real}}) as shown in Fig.\ref{figFieldPipeline}(a).

Instead of for every time, solving the RBF coefficients with the full set of markers, we propose to utilize an MLP to learn the relationship between the simulation field and the function space. That is to say, function space variables $\bm{\gamma}$ are learnable. With the predicted function variables for the RBF from the network, we can establish the mapping between the simulation field and the real field by Eq.\ref{equRBF}.

What's more, the input of our RBF Field Sim2Real transfer network doesn't take the whole surface shape as input. Instead, a single query point $\mathbf{q}_{s}$ (on the simulation surface in the simulation field), along with the predicted function variables to output the calibrated point $\hat{\mathbf{q}}_{s}$in the real field. 

Then, our proposed Sim2Real network will constitute the transferred model by interpolating the real field by traveling the whole simulation surface in the simulation field by Eq.\ref{equRBF}. This architecture gives up the strict requirements of training for the surface input with fixed DoFs, naturally solving the partial information loss problem in \textit{\textbf{the first requirement}}.

Note that this field learning architecture gives up directly learning the mapping between the simulation field and the real field using MLP (we name this as  \textit{\textbf{Naive Field Learning for Surface Sim2Real}} as shown in Fig.\ref{figFieldPipeline}(b)). Instead, we learn the simulation field to function space (Fig.\ref{figFieldPipeline}(a)), which is the physical prior imposed in training, enabling our Sim2Real pipeline to learn not only smooth shapes (considering this representation the radial basis function guarantees at least $C^2$ continuity) but also accurate transfer results (\textit{\textbf{the fourth requirement}}) with a small dataset from hardware (\textit{\textbf{the first requirement}}). The function space is parameterized by the network and, once learned, can be generalized to a sequence of unseen cases (\textit{\textbf{the second requirement}}).

In conclusion, our RBF Field Sim2Real transfer is added at the end of the neural deformation model (on the physical platform) to make the predicted shape more realistic by narrowing the reality gap. It's worth noting that our Field Sim2Real transfer is differentiable, allowing for end-to-end gradient computation through the back-propagation of \textit{\textbf{Space Warping Function}}, \textit{\textbf{B-Spline Surface Function}}, and \textit{\textbf{the RBF Coefficient Prediction Network}} (Further details are provided in Appendix.\ref{Appendix:GradCompShapeLoss} 
\& \ref{Appendix:GradCompNerualDef}). This capability not only fulfills \textit{\textbf{the third requirement}} but also facilitates analytical gradient calculation of the neural deformation, making the proposed FastIK solver (on the physical platform) a reality.


==> tex_GXF/NNFK_IK.tex <==
\section{Preliminary: Numerical Simulator, NN-based FK Model, and IK Solver}
\label{secNNBasedFKIK}

\Guoxin{Modified Jan 25 --- Fig. 2 should be updated accordingly to the updated content.}

In this section, we first present the problem formulation and solution of shape matching as IK problem in the virtual platform as preliminary of the study. A neural network (NN) based method to provide both forward shape prediction of freeform surface using dataset generated by a fast geometry-based simulator. Then the introduction of inverse kinematics computing algorithm using NN-based gradient estimation is follows.

\subsection{Geometry-based numerical simulation for freeform surface}~\label{subsec:simulator}

The starting point of our computation is to build a geometry-based simulator to generate a virtual shape data set $\{ \textbf{a}_k, \mathcal{S}_k \}_{k = 1,2, ... N}$ that captures the connection between the actuation parameter $\mathbf{a}$ and the shape of the free-form surface $\mathcal{S}$. Since the SoRo-Mannequin design contains chambers that to have large expansion, and complex interaction between chambers and outskin, direct apply commercial finite element analysis software (e.g., Abaqus) for this task suffers from high nonlinearity in deformation therefore can be time-consuimg and meet convergence issue. Here we improve the geometry-based simulator presented in our previous work~\cite{Guoxin2020TRO,Guoxin2022IROS} to run the numerical computation. 

The detailed explanation of the proposed computation process is presented in Fig.~\ref{figDataPreparation}(a). It can be seen that we model each pneumatic-driven chamber $\{\mathcal{M}, \mathcal{E}\}$ using a hybrid model where the out layers are modeled using a triangle mesh $\mathcal{M}$ and the inner chamber region is modeled using solid tetrahedral mesh $\mathcal{E}$. During the simulation, we tried to optimize geometry-based elastic energy for each element 
\begin{equation}
    E_{ge} = \sum_{e\in \{\mathcal{M, E} \}} \omega(e) \cdot \|\mathbf{N}(e)\mathbf{V}(e_0) - \mathbf{RN}(e)\mathbf{V}(e)\|_F^2
\end{equation} 
and set the pneumatic actuation as a constraint 
\begin{equation}
    \mathcal{C}_{act}(a) = \sum_{e\in\mathcal{E}}\mathit{Vol}(e) -p(a) \cdot \sum_{e\in\mathcal{E}}\mathit{Vol}(e_0) \equiv 0
\end{equation}
where e is an element (could be a triangle face or a tetra) in the computing space,  $p$ is the volume expansion ratio of the i-th chamber and as a function with the pressure $a_i$ (i.e., $p(a_i)$) to be calibrated in the physical setup. For the chamber that are interact with their neighbors, the interaction-aware energy function based on 'virtual' spring elements (detail presented in~\cite{Guoxin2022IROS}) is included to avoid the interaction between chambers. Same collision response model is also applied to compute the shape of outer skin as a single triangle mesh layer $\mathcal{M}_{skin}$, where the energy $E_{ge}(\mathcal{M}_{skin})$ is minimized and subject to collision constraint applied to compute deformed shape as $\mathcal{S}(\mathbf{a}) = \mathcal{M}_{skin}^d$.

Based on our experiment this geometry-based simulator performs well in generate shape data, which contains similar precision (details are presented in Sec. xx) while greatly imporve the convergence speed compare with Abaqus FEA simulation by xx times (\Tian{Do we need to provide this info?}). We randomly apply the actuation and apply this to a shape data set with data number $N = 1000$ for the FK training purpose.

\subsection{NN-based FK network with B-spline surface control point}

While the numerical simulation provide an effective solution to predit the shape of freeform surface (described by triangle mesh) with given actuator, apply it to estimate the gradient of inverse kinematics computing using numerical gradient can still be slow~\cite{}. To effectively compute shape parameter, here we present a NN-based network for the forward kinematics, where multi-layer perceptron (MLP)-based network $\mathcal{N}_{fk}^{sim}$ is applied to fit the FK function. Unlike reference work in soft robot research where they are typically interested in the task space with end-effector status (generally in dimension $\mathbb{R}^3$), if we feed the shape data as triangle mesh (i.e., $\mathcal{S}_k \in \mathbb{R}^{3m}$, m is the number of vertex), the result training process will be slow and hard to converge as we only have limited number (in our case $N = 1000$) of shape data generate from the numerical simulation. 

In this work, we invite 3D shape parameterization and B-spine surface fitting for the mesh (illustrated in Fig.~\ref{figDataPreparation}(b)) and get control points as the learning parameters of the network\Tian{Need to check}. In our case, we first apply B-spline fitting to get the function
\begin{equation}
    \mathcal{B}(u,v) = \sum_{i=0}^m \sum_{j=0}^n N_{i,p}(u) \cdot N_{i,p}(v) \mathbf{p}_{i,j}
\end{equation}
as another expression of $\mathcal{S}$, where the spline surface control points $\mathbf{p}_{i,j}$ are determined by solving a least-square problem~\cite{}. For all point $v \in \mathcal{S}$, we could find a pair of corresponding 2-dimensional parameters that map to the coordinate as $(u_v, v_v) \rightarrow \mathbf{p}_v = [x_v, y_v, z_v]$. The parameterization is implemented by the as-rigid-as-possible method developed in~\cite{Liu2008localGlobalMeshPara} and can be seen in Fig.~\ref{figDataPreparation}(c), where we cut the mesh by polyline (defined with geodesic distance~\cite{Vitaly2005FastGeodesicDis} between endpoints, highlighted by red color) to release the streatch for a uniform parameterization. It's worth mentioning that for each point on the surface, we can find the UV parameter, and this is important in the sim-to-real process to find correspondance between tracking point on the simulated model (detail presented in Sec. xx). For the B-spline surface, the shape is controlled by control point set $\{ \mathbf{p}_{i,j} \} \in \mathbb{R}^{3mn}$, which have greatly lower dimension than the original $\mathcal{S}_k$. We then put the control point as the output layer of $\mathcal{N}_{fk}$ for the learning and set the loss function as 
\begin{equation}
    \mathcal{O}_{fk} = \sum_{p_i\in\mathcal{S}(a_i)}\| p(a_i) - \mathcal{B}(\mathcal{N}_{fk}^{sim}(\mathbf{a}_i), u_p, v_p)  \|^2
\end{equation}
In this way we build a fast evaluation of FK function by network forward propagation. It's worth mentioning that the network-based surface evaluation is differentiable and the gradient can be directly calculated from network back-propogation to use in IK computing.

\subsection{Fast IK Solver with NN-based Gradient Estimation}

In the virtual platform, the problem of Ik computing is defined as given a target shape $\mathcal{S}^T$, how to find the proper actuation parameter $\mathbf{a}$ that minimizes shape difference defined as

\begin{flalign}\label{eqLoss}
\arg \min_{\mathbf{a}} \mathcal{O}_{\mathit{diff}}(\mathbf{a}, \mathcal{S}^T) & = D(\mathcal{S}^T, \mathcal{S}(\mathbf{a})) \\ & = \sum_{\mathbf{p}_j\in\mathcal{S}} \left\| \mathbf{p}_j - \left(\mathbf{R} \mathbf{c}^{T}_j + \mathbf{t} \right) \right\|^2
\end{flalign}
where the rotation matrix $\mathbf{R}$ and translation vector $\mathbf{t}$ is applied to the target model to eliminate the effect of orientation position, and $\mathbf{c}^{T}_j$ is the closet vertex of $\mathbf{p}_j$ on the target shape $\mathcal{S}^T$.

While this objective of shape difference $\mathcal{O}_{\mathit{diff}}(\mathbf{a}, \mathcal{S}^T)$ can be quickly evaluated by $\mathcal{\mathcal{S}(\mathbf{a})}$ with the trained $\mathcal{N}_{fk}$, it presents high non-linearity in terms of actuation parameter $\mathbf{a}$. Here we propose an gradient-based solver to address the optimization issue, and thanks fully the gradient of the objective function can be analytically computed with the help of network gradient and chain rules as
\begin{flalign}
   \nabla_{\mathbf{a}} \mathcal{O}_{\mathit{diff}} = \frac{d\mathcal{O}_{\mathit{diff}}}{d\mathbf{a}} & = \sum_{j=1}^n 2(\frac{\partial \hat{\mathbf{p}}_{j}}{\partial \textbf{a}})^{T}(\hat{\mathbf{p}}_j - \mathbf{c}^{\mathcal{T}}_j) \\ & = \sum_{j=1}^n 2(\frac{\partial \hat{\mathbf{p}}_{j}}{\partial \textbf{a}})(\frac{\mathcal{B}(u,v)}{\partial \textbf{a}})^{T}(\hat{\mathbf{p}}_j - \mathbf{c}^{\mathcal{T}}_j) ... 
\end{flalign}
\Guoxin{Equation with chain rules to be updated.}

The analytical evaluation of the gradient using network-based FK function is key to the fast iterative-based IK solver, which avoids the time consuming and unstable profess or numerical difference either in simulation platform~\cite{Guoxin2020TRO} or from physical setup~\cite{Tian2022SoRoMannequin, Yip2014TROHardwardGradient}. We apply line search with gradient decent solver in IK computing, and can achieve fast IK solving speed (details presented in Appendex I\Tian{to fill}). In the following section, we introduce the sim-to-real transfer based on field-learning to provide the solution for both FK learning and IK solver in physical setup, maintain same computation efficiency and highly reduce the sim-to-real error in shape matching.




==> tex_GXF/Result_new.tex <==
\section{Implementation Details and Results}\label{secResult}

In this section, we first introduce the design and fabrication process of the SoRo-Mannequin II prototype as the hardware to verify the performance of the proposed fast IK method. Then the implementation details of forward simulation, FK learning process, as well as the NN-based field learning will be presented. After that, the result of continuous forward free-form surface shape prediction and fast IK computing within CAESAR dataset will be presented, the comparsion on the robustenss and effectiveness of proposed field-based sim-to-real learning pipeline will be provided.


\subsection{Hardware System for Verification}

The hardware applied to test the effectiveness of our fast sim-to-real IK computing contains a soft robotic mannequin that contains both the front and back side of human, a closed-loop pressure control system, and vision devices to monitor the shape for verification.

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figFab.jpg}
\caption{Fabrication Steps of the soft robotic mannequin: (a-b) We design, fabricate, and seal a sequence of molds to create a tightly enclosed space. Within this space, liquid silicone is injected, and after a few hours, it transforms into a cohesive soft layer (c-d). For the outer membrane, three molds (one inner mold and two outer molds) are created to be injected with silicone. After consolidation, it will be attached to the top of the mannequin to form the overall shape. 
}\label{figFab}
\end{figure}

\subsubsection{Design and Fabrication}
Our soft robotic mannequin has a three-layer design with an inner soft chamber layer (which can be deformed by pressurized air) attached to base solid chambers, a middle soft chamber layer attached on top of the inner layer (which can also be inflated), and a top membrane layer (passively morphed) covering the base layers to form the overall smooth shape. By actuating the inner and middle layers by pumping air inside the chamber \cite{Tian2022SoRoMannequin} to different pressures, the soft robotic mannequin will be deformed (Fig.\ref{figTeaser}) into different shapes. The fabrication steps are illustrated in Fig.\ref{figFab}. The basic idea of the fabrication is to cast silicone into the spare space enclosed by our carefully designed molds. For the inner layer with 14 chambers, we designed 8 molds (shown in Fig.\ref{figFab}(a)), which will form the empty space before silicone casting as shown in Fig.\ref{figFab}(b). By injecting the liquid silicone (Dragon Skin 20~\cite{DS20}) from the lowest point to the highest point, a group of soft chambers with 2 mm thickness will be fabricated after 4 hours of curing as shown in Fig.\ref{figFab}(c). For the middle soft layer, we seal the two soft membranes to form the inflatable bag and attach it to the first layer as shown in Fig.\ref{figFab}(d). For the top layer of the outer membrane, we designed one inner mold and two outer molds, which will form the space (Fig.\ref{figFab}(f)) to be cast silicone Ecoflex 00-30 \cite{EC30} inside. Finally, after acquiring the consolidated membrane, we have attached it to the top of the base and middle layers to form the mannequin with a soft and deformable free-form surface (Fig.\ref{figFab}(h)). For more details for the casting, please refer to \cite{Tian2022SoRoMannequin}.


\subsubsection{Actuation and Vision System}
During experiments, to achieve controlled pneumatic actuation, we have built an open-source pneumatic platform called OpenPneu (\cite{tian2023openpneu}), to provide multi-channel controlled pressure. It can be easily operated by sending target pressures through serial communication. To get the ground-truth information for our RBF field Sim2Real transfer network and FastIK solver, two vision devices are utilized as shown in Fig.\ref{figTeaser}, including Vicon motion capture system\cite{Vicon} (which will be used to collect marker locations on the deformable mannequin, which is processed to be dataset for Sim2Real network training) and Artec Eva Lite scanner, a structured-light-based scanner\cite{Scanner} to collect scanned ground-truth mesh of the surface to verify the Sim2Real and FastIK results.



\subsection{Details of learning networks $\mathcal{N}_{fk}^{sim}$ and $\mathcal{N}_{field}$}
\label{secLearningSimFKExperiments}

Here we present the details of learning process of two networks. We design the network $\mathcal{N}_{fk}^{sim}$ with two hidden layers, each layer contains 128 neurons. The activation function is select as xx, and we apply xx method for back-propergation. As mentioned before, the input layer contains actuation parameter as vector $\mathbf{a}\in\mathbb{R}^9$, and the output layer is the position of control point, which is also expanded as a vector $\mathbf{p_c}\in\mathbb{R}^{3mn}$. In our implementation we select $m = xxx$ and $n = xxx$, which is suffecient to reconstruct the shape of freeform surface by B-spline fitting. As mentioned in Sec.~\ref{subsec:simulator}, we generate a virtual shape dataset contains $N = 1000$ shapes, and we use the ratio of $7:2:1$ for training, validation, and testing purposes, corresponding. \Guoxin{Here mention our simulation is learning the delta control point difference rather than the real control point.}

For training the field-learning network for robust sim-to-real with limited physical data points, the input layer is ??? and the output layer is the parameter of RBF field $\gamma \in \mathbb{R}^{3(4+N)}$. we set the network structure with xx hidden layer with each layer contains xx neurons. For training the $\mathcal{N}_{field}$, we only have limited data points generated using motion capture system with 50 frames, and each frame contains 18 markers, therefore we did xxx operation of the data points, feed it in a batch to minimize the loss function $\mathcal{O}_{field}$ defined in Eq.~\ref{}.

We implement both network on Pytouch pipeline and trained on a graphics card of xxx, and we set the batch size as xx, the learning rate at xx, and the maximum number of epochs as xx. Cross-validation is applied? and xx backpropagation is employed? For the interference phrase we transfer the trained network and integrated with our IK solver implemented in C++ running in CPU (model xxx). The gradient of the network is computed using xxx.

% \begin{figure}[t] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figSimRepComp.jpg}\\
% \vspace{-2pt}
% \caption{Our simulation FK network is based on MLP to learn the mapping between actuation parameters and surface deformation, which can be described as three different kinds of representation: vertex-based, control-points-based, and delta-control-points-based. We have tested the performance of these representations in the test set (need to show the dataset) and the results are drawn in (a) $\&$ (b). The representation of spline control points can achieve much better accuracy than the vertex-based representation. Furthermore, the delta control points, which are calculated by offsets from the undeformed control points, show even superior performance.}\label{figSimRepComp}
% \end{figure}


\subsection{Result of FK with robust sim-to-real}



We first present the result of forward shape prediction on both virtual platform (predicted with only $\mathcal{N}_{fk}^{sim}$) and physical setup (after applying sim-to-real transfer). In the virtual platform, with the given actuation parameters that never included in the training data, and using the learned control point to reconstruct the surface, we could reach a average surface error (defined as point-to-mesh distance error) at 0.04 mm~\Guoxin{this data to be updated}, which shows the data number and our FK learning with B-spline fitting can well capture the connection between $\mathbf{a}$ and $\mathcal{S}$. Here the surface error is computed by 
\begin{flalign}
    E_{shape}^{avg} (\mathcal{S}_0, \mathcal{S}_1) &= \frac{1}{N} \sum_{k=1}^N \| p^s - p^r \|_2. \\
    E_{shape}^{max} (\mathcal{S}_0, \mathcal{S}_1) &=  \sum_{k=1}^N \| p^s - p^r \|_\infty.
\end{flalign}
However, when compare with the ground-truth shape of mannequin on physical setup $\mathcal{S}^{scan}$, it shows a point-to-mesh distance error at average $E_{shape}^{avg} = 4.99 mm$, and maximum error $E_{shape}^{max} = 21.11 mm$. This high surface prediction error comes from the 'reality gap' where the proposed simulation cannot fully capture the physical properties of soft material. After apply the sim-to-real network with field learning (i.e., apply a field-wapping function with learnied parameter $\gamma$), and compare the difference between $ \mathcal{S}^{real}(a) = \Phi(\mathcal{B}(\mathcal{N}_{fk}(s)), \mathcal{N}_{field}(a))$ and $\mathcal{S}^{scan}(a)$ we get the error reduced by xx, and xx correspondingly with a resulted $E_{shape}^{avg} = xx mm$ and $E_{shape}^{max} = xx mm$. Meanwhile, as high effectivenss of the forward propergation of network, we can continuouly predict the shape of freeform surface and all comes very close with the real physical setup. The result can be found in Fig.~\ref{} and Supplemental Video attached with this manscript.

\Guoxin{below are the description of the new experiment discussed on Jan 25 meeting}
\textcolor{red}{A new figure need to be added here together with the video.}
The result of forward shape estimation shows the robustness and effectiveness of our sim-to-real transfer pipeline, where only 2 mins are used to collect data. As discussed before, we take all 50 frames (average 3.6s/frame) regardless of it contains full set or not to the learning - which is supported by our RBF-based learning pipeline where the information from single point in one frame can contribute to elimate the reality gap. We apply a comparsion on the robustness and effectiency on this hyperthesis, which is illustrated in Fig.xx - where we compare the shape error between two strategy: 1) only apply those frame with all the point being captured; 2) all the point are putting inside. It can be see that from the first few frame, the learning with strategy 1 enables the maximum error decrease sharply - as it contains information in all the set. However, as the time goes and more data from the inperfect frame coming inside, the strategy begin to outperform and give the lowest shape prediction error (in both $E_{shape}^{avg}$ and $E_{shape}^{max}$). This shows the robustness and importance of the proposed field-learning in those case where limited and inperfect data set can only be generated. The corresponding description is also shown in supplemental video.


\subsection{Result of IK Computing}\label{secIKResults}

\begin{figure*}[t] 
\centering
\includegraphics[width=1.0\linewidth]{figure_GXF/FKResult.jpg}
\caption{Result of free-form surface shape prediction using learned network with sim-to-real transfer, which provide a continuous prediction of the shape based on input control parameters.}\label{fig:FKResult}
\end{figure*}

To validate the performance of the gradient-based IK computing to match target shape, we experiment with applying remarkable shape $\mathcal{S}^{taget}$ on the CAESAR dataset \cite{}, and take 100 representative models (based on the height, length of chest line and waistline). For all experimnet we set the terminal condition of iterative-based algorithm as 
\begin{equation}\label{eqTerminalCond}
\frac{|D(\mathcal{T},\mathcal{S}(\mathbf{a}_{i+1}))-D(\mathcal{T},\mathcal{S}(\mathbf{a}_i))|}{D(\mathcal{T},\mathcal{S}(\mathbf{a}_{i+1}))} \leq \tau
\end{equation} 
with $\tau=1\%$ are used in this paper.

The progressive results have been visualized in Fig.\ref{figIKResult} for 100 models, and we first study the convergence curve of the IK computing. The error curve has been plotted to show the whole iteration process. To have a better illustration for the free-form surface shape approximation during iteration, we have drawn two wireframes (red to represent the deformed shape by our Neural Deformation Model and blue to demonstrate the target model with its transformation matrix adjustable) for Iter $\#1$, Iter $\#5$ and Iter $\#30$. These figures vividly demonstrate the success of our Neural network-based IK solver in approximating the provided target shapes, incorporating relative poses in the iterative process. Notice that the comparison models are all captured in physical setup with the scanner. A final converged shape has been scanned and visualized by error colormap by finding its closest distances to the target mesh. The colormap has an average error and maximum error at about 6.16 mm and 22.97 mm respectively. It can also be seen that if we apply the IK solver without apply the sim-to-real transfer the obtained actuation (from FastIK without Sim2Real) showed the worse fit compared to the one with Sim2Real, with an error at xxx, which can due to the gradient elstamtion and shape prediction contains error, and can be seen in Fig.\ref{figIKwithoutSim2RealResult}. As shown in Fig.\ref{figAllResults}, our FastIK solver can achieve a nice approximation to different target models with a large variation in body dimensions. The average error and maximum error for each approximation task can be found in Table.\ref{tab:IKstatistics} (unit is mm).

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figProgressiveResult.png}
\caption{The Progressive results by the proposed Fast IK Solver: The whole process is plotted with three intermediate iterations to validate our algorithm. We further scanned the deformed surface and compared it to the target model with error colormap to verify the correctness of our Sim2Real learning and FastIK solver.\Tian{figure updated}
}\label{figIKResult}
\end{figure}

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figFastIKwithoutSim2Real.jpg}
\caption{We conducted an ablation study to confirm the significance of our Sim2Real method in enhancing the FastIK results. The simulation struggles to well capture real deformation caused by manufacturing imperfections and simulation nonlinearity. However, our Sim2Real method effectively addresses this challenge, further facilitating precise shape approximation to the target model $M3$.\Tian{Discuss about whether we should put histogram here}
}\label{figIKwithoutSim2RealResult}
\end{figure}

\begin{figure*}[t] 
\centering
\includegraphics[width=1.0\linewidth]{figure_GXF/IKResult.jpg}\\
\caption{The final results of approximating four different target models by a side-by-side comparison.\Tian{to-update soon}
}\label{fig:IKResult}
\end{figure*}

\begin{table}[t]\footnotesize
\centering
\caption{The error colormap of the final results. (unit: mm)}
\scriptsize %\tiny \scriptsize \footnotesize \small
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Models:} & $M1$ & $M2$ & $M3$ & $M4$ \\ 
\hline\hline
\textbf{Average Err.: $\frac{1}{n}\sum_{j=1}^n \| \mathbf{p}_j - \mathbf{c}^{\mathcal{T}}_j \|$} & $3.85$ & $5.72$ & $6.16$ & $5.25$ \\ 
\hline 
\textbf{Max. Err.: $\max_{j=1, \ldots, n} \| \mathbf{p}_j - \mathbf{c}^{\mathcal{T}}_j \|$} & $16.37$ & $23.24$ & $22.97$ & $17.68$ \\ 
\hline 
\end{tabular}
\label{tab:IKstatistics}
\end{table}

We also compare the computational time of the IK solver, To assess the efficiency of the proposed FastIK solver in comparison to our previous model-free method \cite{Tian2022SoRoMannequin}, we conducted several experiments to compare the time consumption using these two methods and collect the data in Table.~\ref{tab:CompStatistics}. From Table. \ref{tab:CompStatistics}, our solver can achieve much more efficient computation in all four target models with efficiency improved larger than two magnitudes. For Model M1, our solver only took 7.9 seconds to reach the converged state, which is 119.7 times faster compared to the baseline method with 945.6 seconds. For M2 and M3, our solver achieved 239.4 and 186.5 times faster than the baseline method respectively. For M4, our method could even achieve 258.8 times faster results. It's worth mentioning that our FastIK solver achieved efficient and robust approximation results in less than 8 seconds, which enables practical shape matching, benefiting diverse application scenarios. 



\begin{table}[t]\footnotesize
\centering
\caption{Time Costs on Physical Platform}
\begin{tabular}{c|c|c|c|c}
\hline\hline
\textbf{Models} & $M1$ & $M2$ & $M3$ & $M4$ \\ 
\hline 
\hline 
\multicolumn{5}{c}{Hybrid Solver (Baseline Method $^\dag$)}\\
\hline 
\# of Steps & $14$ & $16$ & $16$ & $20$ \\ 
\hline 
Total Time (sec.) & $945.6$ & $1125.3$ & $1044.6$ & $1242.1$ \\ 
\hline 
\hline 
\multicolumn{5}{c}{Fast IK Solver with Robust Sim2Real Network (Proposed Method)}\\
\hline 
\# of Steps & $14$ & $8$ & $9$ & $8$ \\ 
\hline 
Total Time (sec.) & $7.9$ & $4.7$ & $5.6$ & $4.8$ \\ 
\hline 
\textcolor{blue}{Order of Improvement (times)} & \textcolor{blue}{$119.7$} & \textcolor{blue}{$239.4$}& \textcolor{blue}{$186.5$}& \textcolor{blue}{$258.8$}\\ 
\hline\hline
\end{tabular}
\begin{flushleft}
$^\dag$ The baseline is the model-free algorithm proposed in our previous paper \cite{Tian2022SoRoMannequin}. Note that $\tau=1.0\%$ and $i_{\max}=30$ are used in this experiment. 
\end{flushleft}\label{tab:CompStatistics}
\end{table}


\begin{table}[t]
  \centering
    %%%%%%%%%%%%%Second include the Table
\footnotesize %\small \footnotesize %scriptsize %\tiny 
%Computation time for a single gradient evaluation of the RBF Field Network. 
\caption{The computation cost (unit: millisecond) of the single shape approximation loss $D$ calculation and its gradient $\frac{\partial D}{\partial \textbf{a}}$ (with respect to actuation $\textbf{a}$) evaluation is collected, which is broken down into seven distinct operations (details are listed in Appendix.\ref{Appendix:GradCompShapeLoss} \& \ref{Appendix:GradCompNerualDef} and Fig.~\ref{figVarRelation}). Note that n is the number of the resampling points on the surface and we chose it to be 1200.
}\label{tab:rbfFieldCompTime}
\begin{tabular}{c|c|c|c|c|c|c|c}  %adjust column number 
\hline \hline                       % two horizontal line
%\specialrule{0em}{2pt}{1pt}         %vertical space
\multicolumn{1}{c|}{\multirow{2}{*}{Type}$^\ast$}  & 
\multicolumn{3}{c|}{Forward Pass$^\dagger$} & 
\multicolumn{3}{c|}{Back Propagation$^\ddagger$} &
\multicolumn{1}{c}{\multirow{2}{*}{Total}}\\ %Small Reality Gap
%\hline

% $^\dagger$ \\
% $^\ddagger$ \\
% $^\star$ \\
% $^\ast$ \\

\cline{2-7}
\multicolumn{1}{c|}{}  & 

\multicolumn{1}{c|}{Times} &  %Mean Error
\multicolumn{1}{c|}{Time} &  %Max. Error
\multicolumn{1}{c|}{Total} &  %Mean Error

\multicolumn{1}{c|}{Times} &  %Max. Error
\multicolumn{1}{c|}{Time} &  %Mean Error
\multicolumn{1}{c|}{Total} &
\multicolumn{1}{c}{}\\
\hline\hline

%first operator
\multicolumn{1}{c|}{\Romannum{1}}  & 

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{11.2} &  
\multicolumn{1}{c|}{11.2} & 

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{22.5} & 
\multicolumn{1}{c|}{22.5} & 
\multicolumn{1}{c}{33.7}\\

%second operator
\hline
\multicolumn{1}{c|}{\Romannum{2}}  & 

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{1.3} &  
\multicolumn{1}{c|}{1.3} &  

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{2.1} & 
\multicolumn{1}{c|}{2.1} & 
\multicolumn{1}{c}{3.4}\\

%third operator
\hline
\multicolumn{1}{c|}{\Romannum{3}}  & 

\multicolumn{1}{c|}{n} &  
\multicolumn{1}{c|}{1.1e-2} &  
\multicolumn{1}{c|}{12.8} & 

\multicolumn{1}{c|}{n} &  
\multicolumn{1}{c|}{1.0e-2} &  
\multicolumn{1}{c|}{12.4} & 
\multicolumn{1}{c}{25.2}\\

%fourth operator
\hline
\multicolumn{1}{c|}{\Romannum{4}}  & 

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{1.6} &  
\multicolumn{1}{c|}{1.6} & 

\multicolumn{1}{c|}{1} &  
\multicolumn{1}{c|}{1.5} &  
\multicolumn{1}{c|}{1.5} & 
\multicolumn{1}{c}{3.1}\\

%fifth operator
\hline
\multicolumn{1}{c|}{\Romannum{5}}  & 

\multicolumn{1}{c|}{\multirow{3}{*}{n}} & 
\multicolumn{1}{c|}{\multirow{3}{*}{7.5e-4}} & 
\multicolumn{1}{c|}{\multirow{3}{*}{0.9}} & 

\multicolumn{1}{c|}{n} &  
\multicolumn{1}{c|}{2.0e-3} & 
\multicolumn{1}{c|}{2.4} & 
\multicolumn{1}{c}{\multirow{3}{*}{17.0}}\\

%sixth operator
\cline{1-1}
\cline{5-7}
\multicolumn{1}{c|}{\Romannum{6}}  & 

\multicolumn{1}{c|}{} &  %empty
\multicolumn{1}{c|}{} &  %empty
\multicolumn{1}{c|}{} &  %empty

\multicolumn{1}{c|}{n} &  
\multicolumn{1}{c|}{5.3e-3} &  
\multicolumn{1}{c|}{6.3} & 
\multicolumn{1}{c}{}\\

%seventh operator
\cline{1-1}
\cline{5-7}
\multicolumn{1}{c|}{\Romannum{7}}  & 

\multicolumn{1}{c|}{} &  %empty
\multicolumn{1}{c|}{} &  %empty
\multicolumn{1}{c|}{} &  %empty

\multicolumn{1}{c|}{n} &  
\multicolumn{1}{c|}{6.2e-3} &  
\multicolumn{1}{c|}{7.4} & 
\multicolumn{1}{c}{}\\

%Total 
\hline
\hline
\multicolumn{1}{c|}{Total$^\star$}  & 

\multicolumn{1}{c}{} &  
\multicolumn{1}{c|}{} &  
\multicolumn{1}{c|}{\color{red}27.8} & 

\multicolumn{1}{c}{} &  
\multicolumn{1}{c|}{} &  
\multicolumn{1}{c|}{\color{red}54.6} & 
\multicolumn{1}{c}{\color{blue}82.4}\\

\hline\hline
\end{tabular}
\begin{flushleft}\footnotesize
$^\ast$  The specific operation as detailed in Fig.~\ref{figVarRelation}.\\
$^\star$ The total time cost of the forward pass and backward pass.\\
$^\dagger$ Forward pass of the specific operation.\\
$^\ddagger$ Backward pass of the specific operation.\\


\end{flushleft}
% %Computation time for a single gradient evaluation of the RBF Field Network. 
% \caption{The computation cost (unit: millisecond) of the single shape approximation loss $D$ calculation and its gradient $\frac{\partial D}{\partial \textbf{a}}$ (with respect to actuation $\textbf{a}$) evaluation is collected, which is broken down into seven distinct operations (details are listed in Appendix.\ref{Appendix:GradCompShapeLoss} \& \ref{Appendix:GradCompNerualDef} and Fig.~\ref{figVarRelation}). Note that n is the number of the resampling points on the surface and we chose it to be 1200.
% }\label{tab:rbfFieldCompTime}

\end{table}




 


==> tex_GXF/Sim2Real.tex <==
\section{Robust Sim-to-Real Transfer by Field Learning with Imperfect Data Points}
\label{secSim2Real}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/figSim2RealDataset.jpg}\\
    \caption{The training dataset for our Sim2Real network only consists of 40 frames. What's more, there exists information loss in some frames as indicated by the red dash line, which can be successfully handled by our Robust field learning framework. What's more, our framework can use only sparse ground-truth information (sparse markers compared to dense control points as surface descriptors) to bridge the reality gap as shown in blue line.}
    \label{fig:enter-label}
\end{figure}

The goal of the sim-to-real process is to eliminate the 'reality gap', where we should get a precise physical shape of the mannequin model $\mathcal{S}_{real}(\mathbf{a})$ from the simulated (i.e., predicted by neural network) surface $\mathcal{S}_{sim}(\mathbf{a})$ with corresponding actuation $a$. An intuitive thought is to collect ground-truth shape data set from the physical setup and train a network $\mathcal{N}_{s2r}$. However, as discussed in Sec.~\ref{subsec:motivation}, obtaining dense physical data for the free-form surface is not applicable with scanning-based data collection process. Differently, we apply a motion capture system to take sparse data (i.e., a set of the position of markers $\{ \mathbf{q}_k \}_{k = 1, 2, ...n}$) from the physical setup as ground truth information to build sim-to-real transfer learning. For a given atuation parameter the collected marker position of k-th marker is remarked as $\mathbf{q}_k(\mathbf{a}) \in \mathbb{R}^3$. In the following section, the marker point is also called the anchor point. However, this is also not perfect solution - for each frame that captured, some marker point have the possibility being lossed or uncorved by the object - leading to missed makers and form imperfect data sets.

The sparseness and imcompleteness of marker set (yet easy to get) lead the development of a robust sim-to-real framework to be presented in this section, where field-learning is introduced to learn the parameters of radial basis function (RBF) as shape warping function. The RBF-guided field provide great smooth interpolation on the freeform surface, therefore can construct the surface using sparse marker point. Meanwhile, it can take great advantage of all data points as input, therefore take usage of point in all frames and contribute to eliminite the reality gap. Meanwhile, the field-learning pipeline is also differentiable, making a semmeless integration to our gradient-based IK solver to compute the target parameter.

\subsection{RBF-based Surface Warping}

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figSpaceWraping.jpg}\\
\vspace{-2pt}
\caption{ 
The space warping $\mathbf{\Phi}$ is built on the Radial Basis Function (RBF). The RBF kernels are positioned on the simulation surfaces as markers $\{\mathbf{q}_{t}\}$, transferring the point $\color{red} \mathbf{q}{sj}$ in the simulation field to the corresponding point $\color{blue} \mathbf{\hat{q}}{sj}$ in the real field through the summation of Gaussian values at the location $\color{red} \mathbf{q}{sj}$. However, a specific $\mathbf{\Phi}{i}$ is only applicable to a particular simulation shape $i$; it cannot be generalized to other simulation shapes, presenting challenges for integration into an end-to-end framework.
}\label{figSpaceWraping}
\end{figure}


In our work, the sim-to-real shape mapping of freeform surface is formulated as a elastic space warping problem~\cite{Charlie2007RBFVolPara} where the field-based mapping function $\Phi(\cdot)$ maps all corresponding points with same $(u,v)$ parameter at surface $q_s \in \mathcal{S}^{sim}$ and $q_r \in \mathcal{S}^{real}$ as
\begin{equation}
q^r = \Phi(q^s) = \alpha_0 + Aq + \sum_{i=0, q_i\in \mathcal{S}^{sim}}^N \beta_i e^{-c\| q - q_i \|^2} 
\end{equation}
where $A = [\alpha_1, \alpha_2, \alpha_3]$. Here the gaussian distribution is the radial basis function which has the property of providing smooth surface interpolation to capture the spatial warping. We remark $\gamma = [\alpha_0, \alpha_1, ...  \beta_i]$ as function space variables, which can be detected by solving a linear system. For a given pair of data $[\mathcal{S}(a)^{sim}, \{q_k^{real}(a) \}]$, it defines a linear system contains $N+4$ equations as a well-determined problem. 

While the RBF-based mapping can build a mapping between marker points, solving function space variable $\gamma$, however, is only feasible for the single simulation surface shape and can not be applied to a sequence of surface shapes (as shown in the left-hand side of Fig.~\ref{figSpaceWraping}), which is particularly important in our neural deformation model since it is expected to learn the whole shape space instead of the single shape point. As a result, we further propose to leverage the power of the network to learn the relationship between simulation shape spaces and function space, facilitating continuous function space variables corresponding to varying simulation shapes.

\subsection{NN-based RBF field learning}

Consider the parameters $\gamma$ in RBF mapping is corresponding to the actuation parameter, we use a NN to learn the mapping as $\gamma(\mathbf{a}) = \mathcal{N}_{field}(\mathbf{a})$. In this way, one point $p^r\in\mathcal{S}^{real}(a)$ with parameter $(u_p,v_p)$ in the physical surface can be estimated as 
\begin{equation}
    \Phi(q^s, \gamma(a)) = \Phi(\mathbf{B}(\mathcal{N}_{fk},u_p,v_p), \mathcal{N}_{field}(\mathbf{a})).
\end{equation}
Consider the data set of physical setup contains $M$ frame, and for the k-th frame it contains $N_k$ feasible point ($0 \leq N_k \leq N_{max}$) without loss of information. Different with the solution which only take the frame with full dataset (i.e., $N_k = N_{max}$) as the training data, we define the loss function for training the network $\mathcal{N}_{field}$ as a point-based solution where
\begin{equation}
    \mathcal{O}_{field} = \sum_{i=1,...k} \sum_{j = 1,2,...m} \| \Phi(q_{i,j}^s, \gamma(a_i)) - q_{i,j}^{r} \|^2
\end{equation}
to allow imperfect frames without full set of marker to join the contribution therefore allows imperfect frame without full set of markers contiribute to the sim-to-real transfer to eliminate the reality gap. This results a high effeciency usage of data generated from all frames. 

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figFieldLearning.jpg}\\
\vspace{-2pt}
\caption{ Our proposed RBF Field Learning Framework firstly learns the relationship between surface descriptor (simulation delta control points) and function space variables by MLP. Then, a field Sim2Real calibrates every single point in the simulation field to the real field by differentiable space warping.
}\label{figFieldPipeline}
\end{figure}

After minimizing this loss energy to get the NN-based field parameter, in the inference phase, we densely sample UV pair (or update the traiangle mesh with corresponding UV parameter) with a given resolution, and therefore can get the predicted shape of a freeform surface with reduced sim-to-real gap and can predict the shape $\mathcal{S}^{real}$ in the physical setup. Based on our test, the average shape error compared with ground truth shape captured by 3D scanner is within x.x mm, only 40 frames (with 16 frames containing incomplete data). The result is presented in Sec.xxx\Tian{Fill this}.

For the IK computing, the predicted point $p_j$ on the physical surface is applied, and thus can lead to a fast evaluation of the objective. Meanwhile the process of RBF-based morphing is differentiable, leading to a analytical form of the variable as
\begin{equation}
\frac{\partial\mathbf{\hat{q}}_{sj}}{\partial \mathbf{a}} = \frac{\partial\mathbf{\hat{q}}_{sj}}{\partial \{\mathbf{q}_i\}} \frac{\partial \{\mathbf{q}_i\}}{\partial \mathbf{c}} \frac{\partial \mathbf{c}}{\partial \mathbf{a}} + 
\frac{\partial \mathbf{\hat{q}}_{sj}}{\partial \mathbf{q}_{sj}} \frac{\partial \mathbf{q}_{sj}}{\partial \mathbf{c}} \frac{\partial \mathbf{c}}{\partial \mathbf{a}} + \frac{\partial\mathbf{\hat{q}}_{sj}}{\partial \bm{\gamma}} \frac{\partial \bm{\gamma} }{\partial \mathbf{c}} \frac{\partial \mathbf{c}}{\partial \mathbf{a}} 
\end{equation}
Details of the forward prediction of shape on physical setup with $\mathcal{N}_{fk}^{sim}$ and $\mathcal{N}_{field}$ is presented in Fig.~\ref{figFieldPipeline}.

==> tex_GXF/conclusion.tex <==
\section{Conclusion}
\Tian{Extension: Consider discussing about the selection of conditioning code Z in the future: control points, latent code or actuation parameters?}

.

.

.

.

.

==> tex_GXF/discuss.tex <==

\section{Discussion}

In this section, we compare the performance between proposed robust sim-to-real transfer strategy with field-based learning with other sim-to-real strategy, showcase the robustness and effectivenss on other method. After that, we discuss the limitation of the proposed method, and potential extension of this pipeline to other robot setup.

\subsection{Comparison between sim-to-real strategies}

\Guoxin{To discuss with Yingjun.}

\begin{table*}[t]
  \centering
    %%%%%%%%%%%%%Second include the Table
\small %\small \footnotesize %scriptsize %\tiny 
\caption{Field Learning Architecture Comparison}\label{tab:fieldLearningComparison}
\begin{tabular}{c|c|c|c||c|c|c|c|c|c|c}  %adjust column number 
\hline \hline                       % two horizontal line
%\specialrule{0em}{2pt}{1pt}         %vertical space
\multicolumn{2}{c|}{\multirow{2}{*}{Learning Architecture}}  & 
% \multicolumn{1}{c|}{\multirow{2}{*}{Type}} &
\multicolumn{2}{c|}{Case \Romannum{1}$^\dagger$} & %Case \Romannum{1}
\multicolumn{2}{c|}{Case \Romannum{2}} &
\multicolumn{2}{c|}{Case \Romannum{3}} &
% \multicolumn{2}{c|}{Case \Romannum{5}} &
\multicolumn{1}{c|}{\multirow{2}{*}{Type \Romannum{1}$^\ddagger$}} &   %$C^{1}$ Continuity
\multicolumn{1}{c|}{\multirow{2}{*}{Type \Romannum{2}$^\star$}} &   %Smoothness
\multicolumn{1}{c}{\multirow{2}{*}{Type \Romannum{3}$^\ast$}} \\ %Small Reality Gap
%\hline
\cline{3-8}
\multicolumn{2}{c|}{}  & 

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{Mean} &  %Mean Error
\multicolumn{1}{c|}{Max.} &  %Max. Error

% \multicolumn{1}{c|}{Mean} &  %Mean Error
% \multicolumn{1}{c|}{Max.} &  %Max. Error

\multicolumn{1}{c|}{} &   %$C^{1}$ Continuity
\multicolumn{1}{c|}{} &   %Smoothness
\multicolumn{1}{c}{} \\

\hline\hline

%\color{blue}\ding{51} & \color{red}\ding{55}
\multicolumn{1}{c|}{\multirow{4}{*}{Naive Field Network}}  & 
\multicolumn{1}{c|}{(A) Recon. + ReLU}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
\multicolumn{1}{c|}{NA}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c}{NA}  \\
\cline{2-11}

\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(B) Recon. + Lip.\,\,\,}  & 
% \multicolumn{1}{c|}{2.53}  & 
% \multicolumn{1}{c|}{11.86}  & 

\multicolumn{1}{c|}{4.32}  & 
\multicolumn{1}{c|}{24.36}  & 

\multicolumn{1}{c|}{3.01}  & 
\multicolumn{1}{c|}{21.93}  & 

\multicolumn{1}{c|}{3.61}  & 
\multicolumn{1}{c|}{32.79}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{red}\ding{55}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}   \\
\cline{2-11}


\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(C) Recon. + Siren}  & 
% \multicolumn{1}{c|}{\color{blue}2.14}  & 
% \multicolumn{1}{c|}{\color{blue}9.33}  & 

\multicolumn{1}{c|}{4.97}  & 
\multicolumn{1}{c|}{24.67}  & 

\multicolumn{1}{c|}{4.02}  & 
\multicolumn{1}{c|}{15.88}  & 

\multicolumn{1}{c|}{4.25}  & 
\multicolumn{1}{c|}{17.99}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}  \\
\cline{2-11}

\multicolumn{1}{c|}{}  & 
\multicolumn{1}{c|}{(D) Recon. + RBF}  & 
% \multicolumn{1}{c|}{2.15}  & 
% \multicolumn{1}{c|}{10.26}  & 

\multicolumn{1}{c|}{7.09}  & 
\multicolumn{1}{c|}{24.80}  & 

\multicolumn{1}{c|}{3.96}  & 
\multicolumn{1}{c|}{15.32}  & 

\multicolumn{1}{c|}{3.75}  & 
\multicolumn{1}{c|}{19.65}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{red}\ding{55}}  \\


\hline \hline   %segmentation line between naive filed & rbf field
\multicolumn{1}{c|}{RBF Field Network}  & 
\multicolumn{1}{c|}{(E)}  & 
% \multicolumn{1}{c|}{2.21}  & 
% \multicolumn{1}{c|}{11.63}  & 

\multicolumn{1}{c|}{\color{blue}4.13}  & 
\multicolumn{1}{c|}{\color{blue}18.70}  & 

\multicolumn{1}{c|}{\color{blue}2.96}  & 
\multicolumn{1}{c|}{\color{blue}14.53}  & 

\multicolumn{1}{c|}{\color{blue}3.57}  & 
\multicolumn{1}{c|}{\color{blue}16.26}  & 
% \multicolumn{1}{c|}{3}  & 
% \multicolumn{1}{c|}{3}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c|}{\color{blue}\ding{51}}  & 
\multicolumn{1}{c}{\color{blue}\ding{51}}  \\
\hline\hline
\end{tabular}
\begin{flushleft}\footnotesize
$^\ddagger$ $C^1$ Continuity: measure whether the shape gradient is continuous on the surface.\\
$^\star$ Local Shape Smoothness (defined by Eq.\ref{eqSmoothness}): measure whether the local shape is changing dramatically.\\
$^\ast$ Small Reality Gap: measure the ability of the specific Sim2Real transfer to reduce error.\\
$^\dagger$ Case I: Apply actuation I to deform the prototype.
Mean and Max.: the mean and the maximum error of the calibrated model to the scanned one.\\
\end{flushleft}


%vertical space
\vspace*{0.0\floatsep}

%%%%%%%%%%%%%Then include Figure
\begingroup
\includegraphics[width=1.0\linewidth]{fig/figFieldPropertyComp.jpg}\\
\captionof{figure}{Experiments to compare the output of different field networks: The first one is to measure the $C^1$ Continuity (Type I) and shape smoothness (Type II). All five baselines and our proposed methods are tested and visualized in  (a). Furthermore, we have tested the ability of different methods to reduce the reality gap (Type III) by measuring their distance to the scanned model and visualizing the error by colormap (red color is 15mm). Three different actuation parameters are applied and the results are illustrated from Case I to Case III (b-d). The mean errors and maximum errors are listed in Table.~\ref{tab:fieldLearningComparison}. In conclusion, our proposed method is the only one to simultaneously satisfy all three requirements.
\Tian{Need Case I to be improved}}\label{figFieldProperty}
\endgroup

% Experiments to test the $C^1$ continuity, smoothness a of the learned field from different field learning networks: (a) (b) (c)}

\end{table*}

% content provided by Yingjun ... 

Here we compare the proposed field-learning method with conventional sim-to-real strategies in reconstruct the shape of free-from surface with high DOFs. We implement a general solution of direct building the mapping function from $\mathcal{S}^{sim}$ and $\mathcal{S}^{real}$ using MLP and latent-space training~\cite{xxxxxxx}, as illustrated in xx. For a fair comparsion, we apply same loss function and activation function as despline in Sec.xx for the conventional network.  

We will undertake a series of experiments to validate the following characteristics: 1) The capability of even a naive field learning network to calibrate simulation nonlinearity and fabrication inaccuracy. 2) The superiority of our RBF field learning architecture compared to the naive field learning architecture. 

We first compare the continuity of the network can captured, as it will highly influence the smoothness of the reconstructed surface shape. We evaluate the smoothness using 
\begin{equation} \label{eqSmoothness}
 S_i = \norm{\nabla \norm{\delta_{i}}}
 = \| \nabla \| \frac{1}{d_i} \sum_{j\in N(i)} (\overrightarrow{V_{i}}-\overrightarrow{V_{j}}) \| \|
\end{equation}
The higher value of $S_i$ indicates a rougher surface, possibly featuring wrinkles.

The naive field learning network encompasses various types based on loss functions and activation functions. The initial baseline employs reconstruction loss (Recon. Loss) as the loss function and ReLU as the activation function. The second baseline involves incorporating an additional Lipschitz regularization (Lip. Loss) term~\cite{liu2022lipLoss} into the total loss during the training process. The third and ultimate baselines use reconstruction loss exclusively, but substitute ReLU with the Siren activation function~\cite{sitzmann2020implicit} and RBF activation function~\cite{nabney2004efficientRBFNN}, respectively. Our proposed RBF Field Network was compared with these four baselines. Firstly, the $C^1$ continuity and smoothness properties of the learned field from these different field learning networks were examined. $C^1$ continuity measures whether the shape gradient is continuous on the surface, while smoothness $S_i$ on the mesh vertex $i$ is defined as the norm of the gradient of the Laplacian~\cite{Sorkine2005Laplacian} norm to approximate the magnitude of surface geometry changes: 

In Fig.\ref{figFieldProperty}(a), we have applied the same actuation parameters on five field learning methods and acquired the output calibrated models. The Naive Field Learning approach, employing only Reconstruction Loss (A), fails to produce a continuous gradient in the output field, evident from the surface wrinkles. For the smoothness evaluation, the surface wrinkles (A) have been faithfully highlighted by the red region in Fig.\ref{figFieldProperty}(a) where the local shape is changing dramatically. It is obvious that the Naive Field Learning approach with additional Lip. Loss (B) is still producing a large unsmooth shape. However, the naive field network with Siren activation function, the naive field with RBF activation function, and our proposed RBF field network are capable of creating fields with similar smoothness. 

 
 Moreover, We applied four distinct actuation parameters to the physical setup and compared the scanned mesh with the output of these five methods to calculate both mean and maximum errors. The summarized results can be found in Tab.~\ref{tab:fieldLearningComparison}, and the error colormaps are detailed in Fig.\ref{figFieldProperty}(b-d) where the maximum value for the color bar is 15mm. The statistics and the colormap show our RBF field network for surface Sim2Real has achieved exceptional performance in all cases, largely reducing mean error and maximum error. 
 
 Furthermore, the properties of these field learning architectures are summarized in Table.~\ref{tab:fieldLearningComparison}. Note that considering the naive field learning network with Recon. Loss can not output the $C^1$ Continuity field, we didn't calculate the mean and maximum error of the output meshes of this network to the scanned models. In conclusion, the proposed RBF field learning network is the only field learning network to simultaneously satisfy all three requirements: $C^1$ continuity, local shape smoothness and small reality gap.

\subsection{The capability of RBF Field Network in Sim-to-real transfer}

For \textit{\textbf{the first requirement}} which asks for the learning framework can deal with a modest dataset from hardware with incomplete frames, the training set for our RBF field learning framework only includes 43 frames as shown in Fig.\ref{figDataset}. What's more, we have plotted the available markers and total markers for each frame to further illustrate the details of information loss. 

\textit{\textbf{The second requirement}} 
asks for the sparsity of the training data. Compared to the dimension of the surface descriptor with 900 control points (equivalent to 2700 DoFs), the dimension of the captured markers DoFs is much lower (around 90 DoFs). We have further plotted the percentage of markers' DoFs relative to surface descriptors' DoFs in Fig.~\ref{figDataset}, which is around 3 $\%$. \textit{\textbf{The second requirement}} also asks for the learned framework can be generalized to unseen case. In Fig.~\ref{figFieldProperty}, for case I to case III, these shapes are related to actuation parameters that are not included in the training dataset, but the MLP has successfully learned RBF function space, which further corrected the Sim2Real transfer with error to scanned model largely reduced.

For \textit{\textbf{the third requirement}} that asks for the Sim2Real pipeline to be in an end-to-end manner, our RBF field network is fully differentiable with its end-to-end gradient derived in Appendix.\ref{Appendix:GradCompShapeLoss} 
\& \ref{Appendix:GradCompNerualDef}. To show the computational cost of the shape approximation loss ($D$) calculation and its gradient ($\frac{\partial D}{\partial \textbf{a}}$) evaluation during the forward pass and backward pass by the chain rule as shown in Fig.~\ref{figVarRelation}, a comprehensive table has been illustrated the detailed time consumption. From the Table.~\ref{tab:rbfFieldCompTime}, the forward pass takes 27.8 ms while the backward pass takes 54.6 ms. It is interesting to note that if we use the finite difference on the network to approximate the analytical gradient, it will take $(9 + 1) * 27.8 = 278.0$ ms, which is nearly 3.4 times that of our analytical one. This table shows the ability of our RBF Field Network to efficiently conduct forward pass and back-propagation to acquire the free-form surface shape and its gradient in an end-to-end manner, facilitating the efficient Sim2Real computation and FastIK solver.

For \textit{\textbf{the fourth requirement}} that asks for smooth and accurate Sim2Real transfer, we have validated these characteristics in Sec.~\ref{secRBFFieldLearningResult} and Table.~\ref{tab:fieldLearningComparison}.


\subsection{Limitation and future work}

\Guoxin{To add the limitation and future work here}
.

.

.

.




==> tex_GXF/intro_new.tex <==
\section{Introduction}
\label{secIntro}

\IEEEPARstart{R}{obotics} deformable surfaces have demonstrated the ability to dynamically adapt their shape and structure in response to programmed commands or environmental stimuli. Prototypes have been developed for interactive surfaces~\cite{Stanley2015CtrlSurf,Je2021ElevateAW,inForm2013UIST}, soft robotics manipulators~\cite{Bryan2019SoRoInterface, chen2015dynamic}, and prosthetics for medical phantoms~\cite{inFORCE2019TEI, koehler2020model}. Another notable application is in the garment industry, where Tian~\textit{et al.}~\cite{Tian2022SoRoMannequin} developed a pneumatic-driven soft robotics mannequin capable of deforming to mimic the front side of the human body. This free-form surface contributes to reducing waste and return rates in the textile industry~\cite{textileReport2017}. Here, we present a free-form surface system with improved design compared to~\cite{Tian2022SoRoMannequin}, ensuring shape morphing function to a wide range of human body shapes on both the front and back sides. The deformable free-form surface is pneumatically driven, and its design and function can be seen in Fig.~\ref{fig:Teaser}(a).

\begin{figure}[t] 
\centering
\includegraphics[width=\linewidth]{figure_GXF/figTeaser.jpg}
\caption{(a) A soft robotics free-form surface prototype capable of mimicking the human body shape, equipped with a fast IK solver for practical application feasibility. (b) Challenges in collecting ground truth data from the physical setup, where The 3D scanner can capture detailed shapes, which however is time-consuming and presents boundary and unknown correspondence issues; (c) Motion capture cameras offer continuous marker tracking ability, but only can capture sparse information and suffer from potential marker loss in a single frame. }
\label{fig:Teaser}
\end{figure}

\subsection{Challenges fast IK computing with sim-to-real transfer}~\label{subsec:motivation}

The effectiveness of computing the actuation parameters $\mathbf{a}$ to drive the shape of the free-form surface (denoted as $\mathcal{S}$) to mimic target shapes (marked as $\mathcal{S}^t$) is crucial for practical applications. This is an inverse computing problem, and the shape control is focused on the configuration space~\cite{george2018control} of the free-form surface, which presents much higher degrees of freedom (DoFs) compared to conventional robotic inverse kinematics (IK) problems that focus on task space. This leads to high computation complexity in both forward shape estimation (i.e., predict $\mathcal{S}(\mathbf{a}))$ and the following inverse kinematics computing. An intuitive solution is to directly get shape data from physical setup~\cite{Tian2022SoRoMannequin, Yip2014TROHardwardGradient} and apply a Jacobian-based iterative solver for the IK solution. However, this approach suffers from high computational costs, and its performance heavily relies on the robustness of shape data collection from the physical setup. 

\Guoxin{Direct mention for the actuation where large deformation happens the marker will be dropped.}

For robotic systems with high degrees of freedom (DOFs), data-driven approaches, especially neural networks (NNs), provide an alternative for kinematics modeling and computing. NNs, trained with extensive shape datasets comprising numerous ground truth data points $[\mathbf{a}, \mathcal{S}(\mathbf{a})]$, can accurately map shapes. However, gathering large volumes of training data from physical setups is often challenging. This has led to the development of sim-to-real transfer methods. In this approach, the NN-based kinematics model is initially trained with a vast virtual dataset derived from simulations. Subsequently, only a limited number of data points, collected from the physical setup, are used to bridge the reality gap. This sim-to-real transfer learning strategy is also adopted in this work to build fast IK solver. Yet, to obtain an effective sim-to-real process, the quality of physical data collected for sim-to-real transfer remains crucial.

Unfortunately, collecting shape data from the free-form surface in complex geometry can be time-consuming and unstable, providing substantial obstacles to developing a fast IK solver using both conventional iterative-based methods or/with data-driven approaches even with sim-to-real transfer. As illustrated in Fig.~\ref{fig:Teaser}(c), the method of using a 3D scanner to capture point clouds can be slow and suffer from uncertain boundary regions and occlusion. Additionally, the scanned shape between time sequences shows no correspondence with each other, requiring pre-processing operators to be applied in IK computing~\cite{kwok2014volumetric}. On the other hand, using a motion capture system can precisely capture the position of markers attached to the free-form surface~\cite{scharff2021sensing}. However, only sparse data can be obtained, representing a reduced order of information on the shape of the free-form surface, and can sometimes suffer from marker loss due to camera view occlusion. The difficulties in data collection on the physical setup make the fast and robust IK solver for the deformable free-form surface unfeasible and less explored.

\Guoxin{I'm not sure if the related work section is still needed.}
While previous studies have explored Sim-to-Real research for robots with a dataset containing frames with dense information \cite{Fei2021ICRASim2Real,liang2023real,Rika2022BaySim2Real} or fixed DoFs \cite{Mehrnoosh2022MarkerSim2Real,Fang2022Sim2Real, Gomes2023Sim2RealTactile, peng2018sim} for training, none of them have touched the concept of Sim2Real transfer for a sequence of soft deformable surface deformation with infinite DoFs by only sparse and incomplete ground-truth information.

In the study of kinematics computing of deformable objects (including but not limited to soft robots and deformable object manipulation), the high degrees of freedom (DOFs) in the configuration space are typically modeled either by reduced analytical models or discrete numerical models (comprehensive reviews can be found in~\cite{Renda2023TROModeling, arriola2020modeling}). Numerical simulation is commonly employed as a general solution for modeling deformable objects with complex shapes and can be adapted to cases with internal actuation~\cite{Guoxin2020TRO} or external interactions~\cite{ficuciello2018fem}. However, high-precision numerical solutions cannot be executed rapidly enough to support fast inverse kinematics (IK) solvers. What's more, numerical simulation invariably exhibits a prediction error compared to real physical performance, a discrepancy often referred to as the 'reality gap'~\cite{}. A widely adopted approach to mitigate this issue is to seek help from the data-driven method, which first collects a dataset using the numerical solution and trains a neural network (NN) to fit the forward shape mapping of the soft object~\cite{}. Subsequently, sim-to-real transfer learning~\cite{Dubied2022Sim2RealFEM, Zhang2022Sim2RealSoRoFish, Iyengar2023Sim2RealCTR, Fang2022Sim2Real} is applied to achieve high precision while maintaining reasonable computation time on a limited physical dataset, for both soft robot and soft object manipulation application~\cite{Fei2021ICRASim2Real, liang2023real, Rika2022BaySim2Real}. With this FK-training and sim-to-real transfer pipeline, the shape can be effectively estimated, and the IK computing can take advantage from the differentiability of the network, which can effectively estimate the gradient of IK objectives to finding the solution~\cite{du2021_diffpd, hu2019chainqueen}. While previous studies have explored Sim-to-Real research for robots with a dataset containing frames with dense information \cite{Fei2021ICRASim2Real,liang2023real,Rika2022BaySim2Real} or fixed DoFs \cite{Mehrnoosh2022MarkerSim2Real,Fang2022Sim2Real, Gomes2023Sim2RealTactile, peng2018sim} for training, none of them have touched the concept of Sim2Real transfer for a sequence of soft deformable surface deformation with infinite DoFs by only sparse and incomplete ground-truth information.

\subsection{Our solution and Contribution}

\begin{figure*}[t] 
\centering
\includegraphics[width=\linewidth]{figure_GXF/pipeline.jpg}
\caption{Our sim-to-real learning pipeline, featuring NN-based FK mapping and field-based transfer, efficiently utilizes incomplete motion camera data to eliminate the 'reality gap'.
}
\label{fig:pipeline}
\end{figure*}

\Guoxin{Discussion on main contribution - Jan 25: while less information obtained by sparse dataset (and also incomplete), it's easy to get many frame with less cost, and this lead to higher sim-to-real accuracy using the invited RBF-field learning. Particle marker point - every frame can contribute to the final result.}

In this work, we implement a robust sim-to-real transfer strategy to facilitate fast FK evaluation of the deformable surface, thereafter assist a rapid IK computation for the control of \textit{SoRo-Mannequin} II. Tackle the challenge of unrobust and sparse physical data given for sim-to-real transfer, an approach includes learning the function space for an implicit field using \textit{radial basis functions} (RBF), which forms a neuron-based representation of shape morphing in high-dimensional deformable surfaces, as depicted in Fig.~\ref{figTeaser}. The RBF function has proven effective in spatial extrapolation capabilities, capturing the shape morphing between shape data of free-form surfaces across both the comprehensive virtual space and the sparse yet incomplete physical space. This approach provides a robust sim-to-real transfer learning that fully leverages the entire physical dataset and can benefit from all the sigle vertex point as input to inflect the whole space warping function $W(\cdot)$. Combined with the FK learning network, we can offer an analytical solution for approximating the shape function's Jacobian, thus enabling fast IK computing for 3D deformable free-form surfaces. This strategy effectively bridges the commonly identified reality gap and addresses the challenges of data generation from the physical setup of the robotic deformable surface. \Guoxin{to highlight that we can obtain single-shoot direct parameters computing to fit target shape with neuron-based FK and sim-to-real assisted IK.}

We conducted tests on the newly developed \textit{SoRo-Mannequin} II setup using our proposed learning-based fast IK solver. The virtual dataset, comprising xx data points, was collected from our rapid geometry-based simulator and then integrated with a physical dataset containing xx data points. Notably, 18 out of 30 data points in the physical dataset had missing marker ground-truth data, yet we still achieved robust sim-to-real transfer results. The accuracy of the system improved, achieving a precision of xx mm (\%xx of the workspace) in shape optimization. On average, the computing time for the IK solution on the physical setup was xxs, which is sufficiently rapid for application in this setup (in comparison, the actuation time is xx).

\Guoxin{Above introduction section rewrite at 29 Dec 2023.}


The technique contributions of this work can be summarized into:
\begin{itemize}
    \item A robust Sim2Real transfer learning framework that takes sparse and even incomplete ground-truth information to bridge the reality gap with implicit field representation and Radial Basis Function (RBF) for soft surface morphing with nearly indefinite DoFs. 
    \item A fast IK solver based on neural networks that solves the surface-to-surface approximation problem with analytical gradient for the soft robotic mannequin.
     \item A robotic deformable soft mannequin system named SoRo-Mannequin II consisting of both hardware and intelligent algorithms is built to validate the robustness and accuracy of our Sim2Real pipeline and Neural network-based IK.
\end{itemize}


\begin{figure*}[h] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figDataPreparation.jpg}\\
\caption{ FastIK Solver (Virtual Platform) is proposed to achieve efficient computation of optimal actuation parameters based on a given target model. It includes a neural deformation model aiming at replacing the time-consuming simulation process and post-processing steps (extract free-form surface descriptors as dimension reduction). This surrogate model provides repaid shape and analytical gradient computation, successfully supporting the efficient computation of FastIK solver.
}\label{figDataPreparation}
\end{figure*}


